InfoNCE Loss Provably Learns Cluster-Preserving Representations

The goal of contrasting learning is to learn a representation that preserves underlying clusters by keeping samples with similar content, e.g. the ``dogness'' of a dog, close to each other in the space generated by the representation. A common and successful approach for tackling this unsupervised learning problem is minimizing the InfoNCE loss associated with the training samples, where each sample is associated with their augmentations (positive samples such as rotation, crop) and a batch of negative samples (unrelated samples). To the best of our knowledge, it was unanswered if the representation learned by minimizing the InfoNCE loss preserves the underlying data clusters, as it only promotes learning a representation that is faithful to augmentations, i.e., an image and its augmentations have the same representation. Our main result is to show that the representation learned by InfoNCE with a finite number of negative samples is also consistent with respect to clusters in the data, under the condition that the augmentation sets within clusters may be non-overlapping but are close and intertwined, relative to the complexity of the learning function class.

==> Experiments.tex <==
\section{Experiments}

\subsection{Synthetic Sparse Coding} 
% Experiment one:

% Classification without augmentations. Any classifier that splits clusters must achieve significant loss on augmentations in those clusters, while perform well on augmentations from cleanly separated clusters.


% how to relate classifiers and representations?

% classifier splitting a cluster <==> representations for points from the same cluster are different. how different? 

% project cifar8 reps onto hypercube and check that they are uniform? check that within each class, each image is mapped to same vertex?
% then d should be only 3.

% with different than 2**d clusters, you still don't split them 



% Ideas for experiments from \cite{wang2020understanding}: show that improving pos and neg terms improves downstream performance



\subsection{RGB Images}

\textbf{Datasets.} COCO-on-Places \cite{} and CIFAR-10. 

\textbf{Augmentations.} 

\textbf{Models.} We experiment with progressively larger ResNets.

Goals:

% - Clusters are uniform in some sense - no two natural clusters mapped to same region 

% - Less complex networks give appropriate number of clusters. More complex networks split natural clusters and have larger downstream sample complexity.

- For all model sizes, positive loss is small and inter-cluster variance is large.

- As model size incresaes, negative loss gets smaller and intra-cluster variance increases. Eventually, downstream performance gets worse.

- Larger temperature for positive term decreases intra-cluster variance and improves downstream performance.


\cite{chen2021intriguing} generalizes the InfoNCE loss to a larger family of losses with alignment and uniformity terms weighted according to a hyperparameter, and noticed marginal improvements in downstream performance by increasing the weight on the positive term.


% todo: see if STL works in any regime
% make sure that larger models get smaller negative loss
% get cifar working. interpolate between STL.


todo: try sigmoid activation on the last layer

==> Spiky Augmentations/Conclusion.tex <==
 \section{Conclusion}

 We study properties of minimizers of the InfoNCE loss optimized over function classes with restricted complexity relative to the complexity of augmentations in the dataset, in realistic settings with disjoint augmentation sets and finite negative samples.  Our results show that such representations are uniform and cluster-preserving in the realizable setting, and must be cluster-preserving if they are close to uniform in the agnostic setting. We believe that our novel analytical tools, namely our stochastic argument for the optimality of representations and our inverse partitioning of the space of images, may be of use for future studies of the InfoNCE loss.


% We do not explore the role of bias induced by the optimization algorithm, although it is feasible that it induces a similar bias as the function class, i.e.
% For instance, it may be the case the that the function class contains representations that can cleanly separate all augmentation sets from each other, meaning that the clusters induced by $\mathcal{F}_c$ consist only of single augmentation sets. However, 
% the set of clean  representations attainable by a particular algorithm may induce a meaningful clustering of the data. We leave future work to study this hypothesis.




==> Spiky Augmentations/Experiments.tex <==
\section{Experiments}

\subsection{Synthetic Sparse Coding} 
% Experiment one:

% Classification without augmentations. Any classifier that splits clusters must achieve significant loss on augmentations in those clusters, while perform well on augmentations from cleanly separated clusters.


% how to relate classifiers and representations?

% classifier splitting a cluster <==> representations for points from the same cluster are different. how different? 

% project cifar8 reps onto hypercube and check that they are uniform? check that within each class, each image is mapped to same vertex?
% then d should be only 3.

% with different than 2**d clusters, you still don't split them 



% Ideas for experiments from \cite{wang2020understanding}: show that improving pos and neg terms improves downstream performance



\subsection{RGB Images}

\textbf{Datasets.} COCO-on-Places \cite{} and CIFAR-10. 

\textbf{Augmentations.} 

\textbf{Models.} We experiment with progressively larger ResNets.

Goals:

% - Clusters are uniform in some sense - no two natural clusters mapped to same region 

% - Less complex networks give appropriate number of clusters. More complex networks split natural clusters and have larger downstream sample complexity.

- For all model sizes, positive loss is small and inter-cluster variance is large.

- As model size incresaes, negative loss gets smaller and intra-cluster variance increases. Eventually, downstream performance gets worse.

- Larger temperature for positive term decreases intra-cluster variance and improves downstream performance.


\cite{chen2021intriguing} generalizes the InfoNCE loss to a larger family of losses with alignment and uniformity terms weighted according to a hyperparameter, and noticed marginal improvements in downstream performance by increasing the weight on the positive term.


% todo: see if STL works in any regime
% make sure that larger models get smaller negative loss
% get cifar working. interpolate between STL.


todo: try sigmoid activation on the last layer

==> Spiky Augmentations/Formulation.tex <==
\section{Problem Formulation} \label{section:formulation}

Our learning task consists of {\em (i)} a pretraining phase -- wherein we are not provided supervised labels but rather only \textit{associations} between images and {\em (ii)} a supervised learning phase in which we are provided (a few) labeled data points, labeled according to some specific downstream task. 
During the pre-training phase, we do not know what the downstream task is. However, we are provided \textit{augmentations} of the raw data points that the learner knows should be classified the same way as the raw data for \textit{any} downstream task. In a sense, the augmentations can be seen as modifying the data in a way that leaves the information contained in the data invariant with respect to the downstream tasks.
% {\color{blue} Modulo sounds a bit colloquial}. 
Ideally, we aim to learn a representation that is invariant to such augmentations so that downstream learning can be statistically efficient. 
For interpretability, we will work in the setting of ``images".

\textbf{Images and augmentations.} 
%To formalize the notion 
The images consist of features that are either important for classification or which function only as irrelevant details. Inspired by \citep{von2021self}, we consider an image generation model that consists of {\em (i)} content variables denoted by $\lc$ which capture innate qualities of the images (e.g., the `catness' of a cat), and {\em (ii)} style variables denoted by $\ls$ which capture the appearance of the image (e.g., `rotation' and `crop' for creating augmentations to an image; `long tail' and `furry' for different natural images of dogs). More precisely, each image $x$ is generated according to $x= \I(\lc,\ls)$, where $\I(.,.)$ is a mapping from the space of content and style variables to the space of images. We assume that the natural images are generated such that their content variables $\lc$ belong to the set  ${C}$ and their style variables $\ls$ belong to the set ${S}_\circ$.

We further consider that there is a set of augmentations $\Lambda$, which is a set of functions mapping natural images to augmented images. 
An augmented image of an image $x$ is denoted $\mathcal{A}(x)$, where $\mathcal{A}\in \Lambda$. We assume that the augmented image preserves the content of the original image, while its style may differ from the original image. More precisely, if the original image is given by $x= \I(\lc,\ls)$, then its augmented image $\mathcal{A}(x)$ satisfies the following property:  $\A(x)= \A(\I(\lc,\ls))= \I(\lc,\ls^+)$ for some  $\ls^+\in {S}$, where the set ${S}$ contains ${S}_\circ$. So the augmented images have possibly different style variables \textit{but the same content variables} as the natural images.
Further, the set of augmented images of the image $x = \I(\lc,\ls)$ is called  its \textit{augmentation set} and is defined as $A(x) := A(\I(\lc, \ls)):=\{ \A(\I(\lc, \ls))| \A\in \Lambda\}$, with all images having equal-sized augmentation sets for simplicity. We typically refer to an image $\I(\lc, \ls)$ as $x$ and its augmentation $\I(\lc, \ls^+)\sim A(x)$ as $x^+$, where, for all sets of images $B$, $\sim B$ denotes a random sample drawn uniformly from the set $B$. 
% {Considering the structure of the augmented images, their content variables $\lc$ belong to the set  $\mathcal{C}$, the same as the original images, while their style variables $\ls$ belong to the set $\mathcal{S}$ which contains the set $\mathcal{S}_\circ$, i.e.,  $\mathcal{S}_\circ\subseteq \mathcal{S}$.}
We let ${D}$ denote the set of all images and their augmentations and  ${D}_\circ\subset{D}$ denote the set of all natural images. 
% For a set of images $B \subseteq {D}$, we define $\|B\|_\circ \coloneqq \mathbb{P}_{x \sim {D}_{\circ}}(x \in B)$ and $\|B\| \coloneqq \mathbb{P}_{x \sim {D}}(x \in B)$. 
% {\color{red} Further, we use $\sim$}
% and $\|C\| \coloneqq \mathbb{P}_{x \sim \text{Unif}(\mathcal{D})}(x \in C)$ for 
% For a dataset $\mathcal{D}$, we use $x \sim \mathcal{D}$ to denote a random sample drawn uniformly from $\mathcal{D}$.
% {\color{red} $\mathcal{D}$  is the set of all images?}



%A \textit{random image} refers to an image generated by a uniformly random choice of content and style variables. 


%As a distribution, $\I$ refers to the distribution over random images. $\C$ refers to the distribution over content variables, and $\uS$ refers to the distribution over style variables.

 



% We consider a model for images $\I$, which takes as input content variables $\lc \in \mathcal{C}$ and style variables $\ls$ to create image $\I(\lc, \ls)$. 

% There is a set of augmentations $\A$, which is a set of functions mapping images to augmented images. That is, given an image $\I(\lc,\ls)$, an augmented image is denoted $A(\I(\lc, \ls))$ for $A\in \A$. We will overload the augmentation notation as follows: $A(\I(\lc, \ls)) = \I(A(\lc), A(\ls))$, so augmentations can effectively be thought of as mapping style and content variables to other style and content variables. In our model, we use the content variables exactly to represent the aspects of the image that are invariant to augmentations, as such, we have $A(\lc) = \lc$. We denote the set of augmentations of an image $\{\I(\lc, A(\ls))|A\in \A\}$ as the \textit{augmentation set} of the image. So these augmented images can be thought of as coming from a different choice of style variables \textit{and the same content variables}. For ease of notation, we will sometimes refer to an image $\I(\lc, \ls)$ as $x$, its augmentation $\I(\lc, \ls')$ as $x^+$. A \textit{random image} refers to an image generated by a uniformly random choice of content and style variables. As a distribution, $\I$ refers to the distribution over random images. $\C$ refers to the distribution over content variables, and $\uS$ refers to the distribution over style variables.

% \textbf{Images and Augmentations. }We consider a model for images $\I$, which takes as input content variables $\lc \in \mathcal{C}$ and style variables $\ls$ to create image $\I(\lc, \ls)$. There is a set of augmentations $\A$, which is a set of functions mapping images to augmented images. That is, given an image $\I(\lc,\ls)$, an augmented image is denoted $A(\I(\lc, \ls))$ for $A\in \A$. We will overload the augmentation notation as follows: $A(\I(\lc, \ls)) = \I(A(\lc), A(\ls))$, so augmentations can effectively be thought of as mapping style and content variables to other style and content variables. In our model, we use the content variables exactly to represent the aspects of the image that are invariant to augmentations, as such, we have $A(\lc) = \lc$. We denote the set of augmentations of an image $\{\I(\lc, A(\ls))|A\in \A\}$ as the \textit{augmentation set} of the image. So these augmented images can be thought of as coming from a different choice of style variables \textit{and the same content variables}. For ease of notation, we will sometimes refer to an image $\I(\lc, \ls)$ as $x$, its augmentation $\I(\lc, \ls')$ as $x^+$. A \textit{random image} refers to an image generated by a uniformly random choice of content and style variables. As a distribution, $\I$ refers to the distribution over random images. $\C$ refers to the distribution over content variables, and $\uS$ refers to the distribution over style variables.

\textbf{Clusters.} A collection of images (natural and augmented) forms a cluster if their content variables are the same; thus, $x = \I(\lc, \ls)$ and $x' =  \I(\lc, \ls')$ belong to the same cluster. We denote the cluster of images with content variable $\lc$ by $\Gamma_{\lc}$, and the natural images within cluster $\Gamma_{\mathbf{c}}$ by $\Gamma_{\mathbf{c},\circ}\coloneqq \Gamma_{\mathbf{c}} \cap D_\circ$. As an example, suppose that the content $\lc$ captures the `dogness' of an image. Then, different images of dogs would have the same content, but have different style variables (e.g., furry, skinny, long ears). Recall that the augmentations of an image also share the same content, but the style might be chosen from a different set (e.g., rotation, cropping, blur). {\color{black} In other words, a single cluster is a union of many augmentation sets since not all style variations within a cluster are captured by augmentations.}


{\color{black} \textbf{Representations and heads.} We consider a function class $\F$ of binary functions, $f(x') \in \{-1, +1\}$, where $x'$ is either an image $x$ or its augmentation $x^+$. This is a function class with bounded expressivity (e.g., a class of functions that can be expressed as the thresholded output of a neuron from a neural network with bounded width and depth). We search over $d$-dimensional representations, denoted by $\G$, such that each coordinate of the representation is an element of $\F$, i.e., $g = (f_1, f_2, \ldots, f_d)$,.  Thus a representation $g \in \G := \F^d$ is simply a concatenation of $d$ binary classifiers, mapping an image $x$ to the vertex of the Rademacher hypercube\footnote{Representations in CL often map to the unit hypersphere \citep{wang2020understanding}. Here, we consider a discretized  version of this output space for two reasons: (1) it allows us to construct a naturally restricted representation function class by extending natural properties of binary classifiers, and (2) it provides a tractable setting for us to show the first results that InfoNCE prefers cluster-preserving and uniform representations with finite samples, as it is still an open problem to determine uniform arrangements of finite points on the unit hypersphere \citep{thomson1904xxiv}.
% (1) it allows for a clear notion of uniformity with finite samples, and (2) provides a tractable setting for us to show the first results that InfoNCE prefers uniform and clean representations with finite negative samples.
}
% Formally, $\G$ is taken to be the $d$-ary Cartesian power of $\F$, 
% i.e., $\G = \F^d.$ 
%Thus, a specific representation $g \in \G$ is of the form  $g = (f_1, f_2, \ldots, f_d)$, which takes input $x'$ as above and whose output is a vertex on the $d-$hypercube
$\mathcal{H}_d = \{-1, 1\}^d$.
% (we misuse the terms `Boolean' and `bit' to refer to the binary set $\{-1, +1\}$). 
Note that each $g \in \G$ denotes only the representation (e.g., the body of a neural network). For downstream tasks, a full  classifier is formed by composing $g$ with a {\em head} $\omega\in \J$ for some class $\J$ of heads (e.g., the final classification layer of a neural network).} 

% {\color{red} add remark explaining why it is reasonable to consider representations on the hypercube?
% {\color{black}
% \begin{remark}[Representations on the hypercube] 
% Representations in CL often map to the $d\!-\!1$-dimensional unit hypersphere. Here we consider a discretized (and scaled) version of this output space for two reasons: (1) it allows for a clear notion of uniformity with finite samples, which is notoriously difficult to attain on the unit hypershere \cite{}, and (2) provides a tractable setting for us to show the first results that InfoNCE prefers uniform and clean representations with finite samples. % can be thought of as NN with final-layer sigmoid activation.
% \end{remark}}

% \textbf{Representations and heads. }We consider a function class $\F$ of {\color{blue} rademacher functions, $f(x) \in \{+1, -1\},$ where $x$ is an image or its augmentation}. This is a function class with bounded expressivity, consider for instance the class of neural networks with bounded width and depth. We search for representations such that each coordinate of the representation is an element of $\F$.  that is $\G$ is taken to be the $d$-ary cartesian power of $\F$, $\G = \F^d$. For $g\in \G$, the full classifier is taken to come from a composition $\omega\circ g$ of this representation and a head $\omega\in \J$ for some class $\J$ of heads.

% \textbf{Images and Augmentations. }We consider a model for images $\I$, which takes as input content variables $\lc \in \mathcal{C}$ and style variables $\ls$ to create image $\I(\lc, \ls)$. There is a set of augmentations $\A$, which is a set of functions mapping images to augmented images. That is, given an image $\I(\lc,\ls)$, an augmented image is denoted $A(\I(\lc, \ls))$ for $A\in \A$. We will overload the augmentation notation as follows: $A(\I(\lc, \ls)) = \I(A(\lc), A(\ls))$, so augmentations can effectively be thought of as mapping style and content variables to other style and content variables. In our model, we use the content variables exactly to represent the aspects of the image that are invariant to augmentations, as such, we have $A(\lc) = \lc$. We denote the set of augmentations of an image $\{\I(\lc, A(\ls))|A\in \A\}$ as the \textit{augmentation set} of the image. So these augmented images can be thought of as coming from a different choice of style variables \textit{and the same content variables}. For ease of notation, we will sometimes refer to an image $\I(\lc, \ls)$ as $x$, its augmentation $\I(\lc, \ls')$ as $x^+$. A \textit{random image} refers to an image generated by a uniformly random choice of content and style variables. As a distribution, $\I$ refers to the distribution over random images. $\C$ refers to the distribution over content variables, and $\uS$ refers to the distribution over style variables.





%% A binary classification task $h \in \mathcal{T}$ is a mapping from the space of images to $\{-1, 1\}$. The set of tasks naturally induce a set of clusters over images. Specifically, two images $x, x'$ belong to the same cluster if for all tasks $h \in \mathcal{T},$ $h(x) = h(x').$ Qualitatively, we expect such clusters to 


%% Given the set of tasks \mathcal{T}, our goal is to learn a rep

\textbf{Goal of pretraining.}
Ultimately, we aim to find a representation that allows for easily solving  tasks from a set of possible downstream binary classification tasks $h \in \mathcal{T}$, where each task $h$ maps an image to a binary label $\{-1, 1\}$.
These tasks are assumed to be faithful to the clusters, meaning that for any pair of images $x, x'$ belonging to the same cluster, $h(x) = h(x')$.

% $\F_c$ as possible. 
Note that during pretraining, the learner does not have any knowledge about which task will be assigned among the solvable ones. After pretraining, the learner fixes the representation but can learn a task-specific head when it encounters a downstream task.
We define the error a representation $g$ on the downstream task $h \in \mathcal{T}$ with respect to the class $\mathcal{J} \subseteq \{\omega: \mathbb{R}^d \rightarrow \mathbb{R}\}$ of allowed heads as
% The error of  $g$ on is 
% with $n$ samples allowed for learning the head is:
   \begin{align}
    \uL_{h,\mathcal{J}}(g) \coloneqq \inf_{\omega \sim \mathcal{J}}\mathbb{P}_{x \sim {\mathcal{D}}}[ \omega \circ g(x) \neq h(x) ]. %_{S,y} 
\end{align}
% where 
% % \begin{align}
% %     \omega_{S,y} \coloneqq \min_{\omega \in \J} \frac{1}{n}\sum_{x \in S} 1{\{\omega \circ g(x) \neq y(x)\}},
% % \end{align}
% i.e. $\omega_{S,y}$ minimizes the empirical loss of $\omega \circ g$ on $n$ labeled samples from the downstream task.
The error of $g$ on a family of downstream tasks $\mathcal{T}\subseteq \mathcal{F}_c$ is the worst case  error among tasks in $\mathcal{T}$:
\begin{align}
    \uL_{\T,\J}(g) \coloneqq \sup_{h \in \mathcal{T}} \uL_{h,\mathcal{J}}(g).
\end{align}
% Our main assumption describes a specific relationship between $\T$ and $\F$ and formalizes the notion of an inductive bias in $\F$ with respect to $\T$: For any function $f\in \F$ satisfying $f(\I(\lc, \ls)) \ne f(\I(\lc', \ls'))$ for $\lc\sim \lc'$, there exists $\lc^{(1)}, \ls^{(1)}$ and $\ls^{(2)}$ satisfying $f(\I(\lc^{(1)}, \ls^{(1)})) \ne f(\I(\lc^{(1)}, \ls^{(2)}))$. In other words, any function in the supervised function class $f\in \F$ that splits a cluster must also split an augmentation set within the cluster.
To summarize, for a task that is realizable \textit{with supervision} using function class $\F$, we would like to learn a representation entirely from unlabelled data such that the task on the embedded images is still realizable for $\J$.
The overall motivation is that learning $\omega\in \J$ can generally require fewer \textit{labeled} samples than learning the joint model $\omega\circ g$. 

% Our objective is to learn a representation $g\in \G$ such that classification of the embedded images $g\circ \I(\lc, \ls)$ results in generalization error comparable to \textit{supervised} classification. Let $y_\ast\in \C$ be a function mapping images to labels in $\{-1,1\}$  for a downstream task. 
% Define the linear classification loss on this downstream task as the smallest classification error that can be achieved by composing a linear classifier with $g$, namely
% \begin{align}
%   \uL_{\text{clf}}(g, y_*) \coloneqq \inf_{h\in \mathbb{R}^d}   \mathbb{P}_{\mathbf{c},\mathbf{s}} (\{y_*(\I(\lc, \ls))  h^\top g\circ \I(\lc, \ls) < 0\}])
% \end{align}
% We aim to learn a $g$ such that $\uL_{\text{clf}}(g, y_*) - \inf_{f \in \mathcal{F}} \mathbb{P}_{\mathbf{c},\mathbf{s}} (\{y_*(\I(\lc, \ls)) f\circ \I(\lc, \ls) < 0\}])$ is small for all ``reasonable'' downstream tasks $y_*$.
% \begin{align}
%     \uL_{rep}(g) \coloneqq \mathbb{E}_{\mathcal{T}}\left[\inf_{h\in \mathbb{R}^d} \uL_{cls}(h,g,\mathcal{T})\right]
% \end{align}

% {\color{red} or $y_*$ is a function of $(\mathbf{c},\mathbf{s})$?} 

% \section{Supervised to Unsupervised: }
%We make the following assumption on the function class. Our goal is to demonstrate unsupervised representation classes $\G$ inherit the biases of their corresponding supervised function classes, and for that we need to formally describe the bias present in the supervised function class $\F$.

% \begin{assumption}
%     The function class $\F$ is such that 
%     \begin{enumerate}
%         \item for any boolean valued function $h:\C\to \{-1,1\}$, there is some $f\in \F$ such that $f(\I(\lc, \ls)) = h(\lc)$.
%         \item for any $f\in \mathcal{F}$, $\min_h \E[f(\I(\lc, \ls))\ne h(\lc)] \not\in (0, \delta]$.
%     \end{enumerate}
% \end{assumption}



% {\color{black} \textbf{Example.} Suppose that we have four classes of images -- cats, dogs, ducks and sparrows -- each with its augmentations (e.g., rotations, crop, blur). Our goal is to find a representation that would enable us to quickly solve for a variety of classification tasks such as `dog vs cat', `bird vs. mammal', and `cat vs non-cat' (denoted by $f \in \T$). Here, $x, x'$ each represents an image or its augmentation, and $x \equiv x'$ means that they both should be classified identically for each of the three classification tasks.}


\subsection{InfoNCE loss}

We denote $\mathbb{E}_{x,x^+} \coloneqq \mathbb{E}_{x \sim {D}_{\circ},x^+\sim A(x)}$ and $\mathbb{E}_{x,x^+, \{x^-_i\}_{\ell}} \coloneqq \mathbb{E}_{x \sim {{D}_{\circ}},x^+\sim A(x), \{x^-_i\}_{\ell} \sim {D}_{\circ}^\ell}$ for simplicity.  The InfoNCE loss we consider is given by\footnote{{
   For ease of exposition
we consider the case wherein negative samples are drawn from the set of {natural images, as in \citep{wen2021toward}.} Although this may not hold in practice, it greatly simplifies the presentation of our results.}}
\begin{align}\label{eq:InfoNCE} %_{\text{SimCLR}}
    &\uL({g}) = -\underbrace{\beta \mathbb{E}_{x,x^+} [g(x)^\top g(x^+) ]}_{\text{alignment}} \;  + \; \underbrace{\mathbb{E}_{x,x^+, \{x^-_i\}_{\ell}}\left[ \log\bigg({ e^{\beta g(x)^\top g(x^+)}\!+\!\sum_{i=1}^\ell e^{\beta g(x)^\top g(x^-_{i})}  } \bigg)\right]}_{\text{uniformity}}
\end{align}
Following \citet{wang2020understanding}, we refer to the first term as the \textit{alignment} term, or the \textit{positive} term, and we refer to the second term as the \textit{uniformity} term or the \textit{negative} term.
By minimizing the first term, we are maximizing the alignment between the representation of an image and its augmentation, and by minimizing the second term we are enforcing the representation of different images to be as different as possible. 


{\color{black}{The above formulation suggests that the representation learned by minimizing the above loss forces images and their augmentations to have a similar representation. What we show in the following sections is a stronger result which guarantees by minimizing the InfoNCE loss, all images that belong to the same cluster (share the same content) will have a similar representation. 
}}
%In the following, we demonstrate an improved understanding of InfoNCE solutions that explicitly invokes the alignment and uniformity properties described in \cite{wang2020understanding}. Specifically, we will show that the positive term ensures that the equivalence relation on images is respected by the representation learned by minimizing the InfoNCE objective. This allows us to realize \text{some} set of downstream tasks. Meanwhile, the negative term encourages the representation to be such that it spans a maximal number of downstream tasks. Taken together, our representation realizes a maximal number of downstream tasks.

%%%%%%%%% Our approach now is as follows. We will first show that contrastive learning using the SimCLR loss learns representations such that each coordinate of the representation cuts the augmentation sets 
% cleanly. Specifically, the positive portion of the SimCLR loss ensures that each of the style clusters are classified the same way by each coordinate learned by SimCLR. We will then show that the negative portion of the SimCLR loss encourages representations which when taken together span the largest possible set of downstream tasks.

% The function class $\mathcal{F}$ consists of functions $f: \mathcal{I} \rightarrow \{-1,1\}$.



% For ease of notation, denote $\mathbb{E}_{x,x^+} \coloneqq \mathbb{E}_{x \sim \bar{\mathcal{I}},x^+\sim \mathcal{A}(x)}$ and $\mathbb{E}_{x,x^+, \{x^-_i\}_{\ell}} \coloneqq \mathbb{E}_{x \sim \bar{\mathcal{I}},x^+\sim \mathcal{A}(x), \{x^-_i\}_{\ell} \sim \mathcal{I}^\ell}$. The InfoNCE loss is given by
% \begin{align} %_{\text{SimCLR}}
%     &\uL({g}) = -\beta \mathbb{E}_{x,x^+} [g(x)^\top g(x^+) ] \nonumber \\
%     &\;  + \mathbb{E}_{x,x^+, \{x^-_i\}_{\ell}} \log\bigg({ e^{\beta g(x)^\top g(x^+)}\!+\!\sum_{i=1}^\ell e^{\beta g(x)^\top g(x^-_{i})}  } \bigg) %\label{simclr}
%     % \uL_{\text{SimCLR}}^{+}({g}) + \uL_{\text{SimCLR}}^{-}({g}) \nonumber \\
%      % \uL_{\text{SimCLR}}^{+}({g})&= \mathbb{E}_{x,x^+, \{x^-_i\}_{\ell}}[ -\beta_1 g(x)^\top g(x^+) + \log() ] \nonumber \\
%      %  \uL_{\text{SimCLR}}^{+}({g})&= \mathbb{E}_{x,x^+, \{x^-_i\}_{\ell}}[ \log(e^{\beta_2 g(x)^\top g(x^+)}+ \sum_{i=1}^\ell e^{\beta_2 g(x)^\top g(x^-_{i})} ) ] \nonumber \\
%     % \mathbb{E}_{\omega \sim \text{Unif}(\bar{\mathcal{I}}), \omega_i^- \sim \text{Unif}({\mathcal{I}})}\left[ \log\left(\frac{\exp(\beta \hat{g}(\omega)^\top \hat{g}(\omega^+))+ \sum_{i=1}^\ell \exp(\beta \hat{g}(\omega)^\top \hat{g}(\omega_i^-))}{ \exp(\beta {g}'(\omega)^\top {g}'(\omega^+))+ \sum_{i=1}^\ell \exp(\beta {g}'(\omega)^\top {g}'(\omega_i^-))  } \right)
%      % \right] \nonumber \\
%  %     &\quad + \beta \mathbb{E}_{\omega \sim \text{Unif}(\bar{\mathcal{I}}), \omega^+ \sim \mathcal{A}(\omega)}[ 
%  % {f}_1'(\omega){f}_1'(\omega^+) - \hat{f}_1(\omega)\hat{f}_1(\omega^+) ] \nonumber \\
% \end{align}

% \subsection{Model Assumptions}
% We now formalize the assumptions that we will work with.

% A downstream task $y: \mathcal{I}\rightarrow \pm 1$ is a mapping from images to a binary label from a set $\T$ of all possible downstream tasks. We assume that all downstream tasks label all images from the same cluster identically, 




% \begin{assumption}{Implementability}
%     If $f\in \mathcal{F}$, then 
% \end{assumption}

% \begin{assumption}{Downstream tasks}\label{assump:downstream}
%     For any downstream task $\mathcal{T}$, labels agree on all points in the same cluster.
% \end{assumption}


% \subsection{SimCLR Leads to Uniform Representations}

% \subsection{Definitions and Assumptions}
% % We conclude this section with a discussion of our assumptions. 
% We conclude this section with some definitions formalizing some of the notions introduced above. The first is that of \textit{cleanness}. A representation is clean if each of its coordinates separate the data cleanly into sets of clusters.
% \begin{definition}[Clean]
% A representation $g\in \mathcal{G}$ is {\em clean} iff $g(x) = g(x')$ for all $x\sim x'$. A classifier $f\in \F$ is {\em clean} iff $f(x) = f(x')$ for all $x\sim x'$. The set of clean classifiers is denoted $\F_c$ and the set of clean representations is denoted $\G_c$.
% \end{definition}
% Our first result will show that when it is possible to split the clusters \textit{cleanly} and \textit{uniformly}, then the representation learned by maximizing InfoNCE is always clean and uniform. Here a \textit{uniform} representation, we mean one such that the push-forward measure onto the hypercube is uniform. 
% \begin{definition}[Uniformity]
% A representation $g\in \mathcal{G}$ is {\em uniform} iff $\Pr_{x\sim \I}(g(x)=v)=2^{-d}$ for all $v\in \mathcal{H}_d$.
% \end{definition}
% \begin{assumption}[Realizability]\label{assump:realizability}
%     There exists a $g \in \mathcal{G}$ that is both clean and uniform.
% \end{assumption}
% In order for there to exist a representation that is both clean and uniform, the semantic clusters in the dataset must be balanced. Although this may seem like a strong assumption, in practice training on unbalanced datasets tends to reduce the performance of models optimized via InfoNCE \cite{assran2022hidden}. 

% When there does not exist a clean, uniform representation, we show that under some different assum

% % \begin{assumption}[old] \label{assump:spiky-full}
% % For any $f\in \mathcal{F}$ and any cluster $C$, let $p(f,C)\coloneqq \min(1-\mathbb{P}_{x_1^- \sim C}[f(x)=1],\mathbb{P}_{x_1^- \sim C}[f(x)=1])$ and $e(f,C)\coloneqq \mathbb{P}_{x \sim \bar{C}, x^+ \sim \mathcal{A}(x)}[f(x)\neq f(x^+)]$. Then for some $\delta\in (0,1]$, a dataset is called $\delta$-spiky with respect to the function class $\mathcal{F}$ if
% % \begin{align}
% %     \delta p(f,C) \leq e(f,C) \leq 2 p(f,C)
% % \end{align}
% % for all $f\in \mathcal{F}, C$.
% % \end{assumption}

% \begin{assumption}[Regularity of $\mathcal{F}$ w.r.t. augmentations] \label{assump:spiky}
% For any $f\in \mathcal{F}$, for all clusters $j\in [m]$, if $f(x)\neq f(x')$ for some $x\sim x'$, then $\exists A, A'\in \A$, $x\in \I$ such that $f(A(x))\neq f(x)$.
% \end{assumption}

% \begin{assumption}[$\gamma-$Regularity of $\mathcal{F}$ w.r.t. augmentations] \label{assump:spiky}
% For any $f\in \mathcal{F}$, for all clusters $j\in [m]$, if $f(x)\neq f(x')$ for some $x\sim x'$, then $\exists A, A'\in \A$, $x\in \I$ such that $f(A(x))\neq f(x)$.
% \end{assumption}

==> Spiky Augmentations/Introduction.tex <==
\section{Introduction}

Representations pretrained on partially or completely unlabeled data are becoming ubiquitous in machine learning applications \citep{DBLP:journals/corr/abs-1802-05365,radford2021learning}, in large part due to the availability of large unlabeled datasets and significant computing power offline, and the effectiveness of self-supervised representation learning algorithms, especially contrastive learning (CL). CL aims to learn representations that treat natural images similarly to their augmentations, while maximizing the average distance between random pairs of images. In recent years CL has demonstrated numerous successes in pretraining representations with unlabeled data that learn meaningful relationships between data points that generalize well to  downstream tasks in computer vision \citep{hjelm2018learning,oord2018representation,bachman2019learning,caron2020unsupervised,chen2020simple,chen2020big,he2020momentum,henaff2020data,li2020prototypical,misra2020self,tian2020contrastive,tian2020makes} and natural language processing \citep{brown2020language,gao2021simcse,su2021tacl,radford2019language}. 

Despite its empirical success, it is not well-understood how CL learns meaningful relationships between data points. Since data are unlabeled, the only immediate structure in datasets leveraged by CL are the sets of images and their augmentations. Without further assumptions, this structure is insufficient to learn relationships between images across augmentation sets.
%
To circumvent this issue there are two approaches. The first is to assume that augmentation sets of semantically similar natural images overlap, i.e. for two images of cats, some of the augmentations of each image are equivalent \citep{arora2019theoretical,haochen2021provable,haochen2022beyond,shen2022connect,wang2022chaos}. However, this assumption is unlikely to hold in practice, as pointed out by recent work \citep{saunshi2022understanding}. The second approach is to consider inductive biases of the representation function class and/or optimization algorithm, and use these to argue that only certain types of representations (that capture semantic relationships) can be learned.

Prior studies have initiated the study of how inductive biases of the representation class can lead to meaningful representations in CL \citep{saunshi2022understanding,haochen2022theoretical}, but their analysis is for the spectral contrastive loss, which is not used in practice. Instead, the vast majority of CL approaches, including the widely popular SimCLR framework \citep{chen2020simple}, optimize a loss function based on the InfoNCE loss \citep{gutmann2010noise,oord2018representation}. A variety of works have studied properties of the InfoNCE loss, but due to its unwieldy log-sum structure have made restrictive assumptions, such as having infinite  \citep{wang2020understanding,robinson2020contrastive,von2021self} or only a single \citep{tosh2021contrastive,huang2021towards} negative sample(s). 

%\subsection{Main Contributions}
%\label{sec:contrib}
\vspace{0.05in}
\noindent \textbf{Main Contributions.} {\color{black} We are given a collection of clusters of natural images, with each image associated with  augmentations (positive samples such as `rotation') and a finite set of negative samples (unrelated images). Using the InfoNCE loss, our goal is to learn a $d-$dimensional representation $g \in \G$, where $g = (f_1, f_2, \ldots f_d)$ and $\{f_i\}$ are binary functions mapping images to $\{-1, 1\}$ (thus $g$ maps images on the {\color{black}  hypercube} $\mathcal{H}_d = \{-1, 1\}^d$).
% , such that when this is composed with a head, can solve all downstream binary classification tasks of interest.   
%
Our setting is one where the function class has bounded expressivity with respect to the augmentation sets, meaning that the augmentation sets within clusters are intertwined, and {hard} to separate from the rest of the cluster using functions in $\mathcal{F}$. }

% is a property both of the (Boolean) function class and the augmentations. It roughly says that 
% if a function splits two natural images in a cluster, then it also splits some image in that cluster from atleast one of its augmentations.

%% (map from images to a vertex on the Rademacher hypercube $\mathcal{H}_d = \{-1, 1\}^d$)

% that inherit this inductive bias, namely, that the function class clusters the images consistent with these downstream tasks. Formally, a representation is a mapping from images to a vertex on the Rademacher hypercube $\mathcal{H}_d = \{-1, 1\}^d$.

\vspace{0.05in}
\noindent \textbf{(Realizable Setting)} Suppose there exists a representation $g^* \in G$ that is: {\em (a)} {cluster preserving, and {\em (b)} different clusters of images are uniformly mapped over distinct vertices on the hypercube
% and furthermore the induced distribution is uniform 
(qualitatively, class-balance in the image dataset). We show that with {\em any finite number of negative samples}, the representation learned by the InfoNCE loss is cluster-preserving and uniform. Furthermore, this learned representation when composed with a two-layer ReLU head, achieves zero downstream error on any cluster-preserving binary classification task. Our proof hinges on a novel Markov Chain construction showing that the InfoNCE loss of any non-uniform representation can be improved by ``blurring'' the representation through the Markov Chain transitions. Conversely, we show that solutions to the InfoNCE loss optimized over an arbitrarily powerful representation class $\mathcal{G}_\star$  cannot have meaningful downstream performance guarantees on such tasks.

%\vspace{0.05in}
%\noindent \textbf{(Agnostic Setting)} In the non-realizable setting with arbitrary numbers and sizes of clusters, we prove  that representations in $\mathcal{G}$ that are close to uniform under a looser notion of closeness must also be clean if they are minimizers of the InfoNCE  loss on $\mathcal{G}$.  Our proof exploits the geometry induced by the inverse maps from the hypercube to the space of images by the pair of representations -- the non-clean map, and a perturbed (potentially cleaner) map. These together induce a partition over the space of images, leading to multiple cases. In each of these cases, we show that the improvement in the InfoNCE loss due to positive samples outweighs the effects of negative samples while moving from the non-clean to the cleaner representation.

%Our proof leverages a novel partitioning of the image space  that may be of independent interest for future analysis of the InfoNCE loss.

\vspace{0.05in}
\noindent \textbf{(Agnostic Setting)} In the agnostic (non-realizable) case, through sensitivity analysis, we show that for any close-to-uniform and non-cluster-preserving representation, there exists a  representation that preserves one additional cluster and thus improves the InfoNCE loss. Our proof uses a novel partitioning of the image space that is of independent interest for future analysis of the InfoNCE loss.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\color{red} Rewrite from here -- In this work, we provide the first study of  how inductive biases of the function class on which the InfoNCE loss is optimized affect downstream performance, without making restrictive assumptions on the number of negative samples used in the loss. In particular, the inductive bias we consider is that for all sets of images that are labeled the same way on all downstream tasks of interest, all representations in the function class $\mathcal{G}$ must either (i) represent each image in each set identically or (ii) represent two images from the same augmentation set within this set differently.
% sets of points that are not split by any downstream 
% }

% OLD:

% The vast majority of  contrastive learning approaches, including the widely popular SimCLR \cite{chen2020simple}, optimize a loss function based on the InfoNCE loss \cite{gutmann2010noise,oord2018representation}.
% % , which is closely related to the SimCLR loss \cite{chen2020simple}. 
% % Despite its popularity, contrastive learning in general, and especially contrastive learning with the 
% % most widely  
% % InfoNCE loss, is not well-understood theoretically.
% Multiple works have shown that InfoNCE losses encourage representations to have two desirable properties: (i) \textit{alignment} -- different views of the same image are mapped to similar points, and (ii) \textit{uniformity} -- the output feature distribution is uniform on some space.
% However, it remains a challenge to rigorously quantify to what extent solutions to the InfoNCE loss satisfy these properties, especially with finite samples, and why satisfying them leads to strong downstream performance. 

% % Early works showed that contrastive loss functions trade off between 
% Recent works have studied CL in terms of its ability to recover clusters of semantically similar images that are likely to share downstream labels \cite{arora2019theoretical,haochen2021provable,shen2022connect,haochen2022beyond}. To show that solutions of contrastive losses recover such clusters, these works consider an unrestricted function class and assume that semantically similar natural images share augmentations, i.e. their augmentation sets are non-disjoint. 
% % It is a mystery why CL yields representations that treat semantically similar images similarly, i.e. images that are likely to have the same label on downstream tasks, while separating semantically dissimilar images, even though no label information is available to convey these semantic relationships.
% % Early works bounded the downstream task error of contrastive representations from unrestricted function classes under the assumption 
% % Early works argued that contrastive learning  generalizes well because   augmentation sets of semantically similar images overlap, thus all functions . 
% However, \citet{saunshi2022understanding} recently observed that such an assumption does not hold in practice, as complex representations can minimize contrastive losses while separating semantically similar images and their augmentation sets -- highlighting the need to incorporate inductive biases of the function class and learning algorithm to guarantee downstream accuracy. Initial works have given downstream guarantees that use inductive biases of the function class to avoid strong assumptions on the augmentation sets \cite{saunshi2022understanding,haochen2022theoretical}, yet these results apply only for the spectral contrastive loss, a stylized loss function that is not used in practice.

% % In addition to understanding how CL effectively captures clusters of meaningfully related images, it is also important to understand how contrastive representations separate disparate images. Ideally, the distribution of represented images should be in some sense uniform to allow for the largest expressivity of downstream tasks \cite{}, and indeed CL seems to yield uniform representations in practice \cite{wang2021understanding}. \citet{wang2020understanding} showed that CL with the InfoNCE loss yields uniform representations on the hypersphere in the limit of infinite negative samples. To the best of our knowledge, no prior work has shown that CL yields uniform representations with finite samples.

% In this work, we study CL with the InfoNCE loss under a natural and general inductive bias on the representation function class inspired by supervised learning. The fundamental function class inductive bias that enables supervised learning is that the complexity of the class is limited such that training error is a good surrogate for test error.
% % that enables supervised learning is the 
% % principal that if a function incorrectly labels points in the underlying input marginal distribution, then it must incorrectly label a commensurate number of points in the training set. Satisfying this with finite training samples induces a bound on the complexity of the function class. 
% We translate this bias to unsupervised CL by restricting our function class to include only functions that satisfy the following property: if they represent some pair of images in the same semantic cluster differently (analog of having test error on this cluster) then they also represent at least one pair of images from the same augmentation set differently (analog of having training error). This is illustrated in Figure \ref{fig:spiky}.
% % Essentially, the function class is not complex enough to split augmentation sets with intricate boundaries, thus these augmentation sets form clusters preserving semantic relationships in spite of the augmentation sets being disjoint.

\textbf{Main contributions.} Our natural assumption on the function class allows us to show that optimal solutions to the InfoNCE objective  are {\em clean} in the sense that they represent all images from the same cluster identically. Moreover, we show that among clean representations, the optimal representation maps clusters {\em uniformly} on the hypercube. Our contributions are further detailed as follows.}
% Although \citet{haochen2022theoretical} recently studied a similar inductive bias, their analysis is limited to a stylized
%% toy 
% loss function not commonly used in practice.
% and their results allow for a number of clusters that scales only linearly in the representation dimension, whereas we allow for exponentially many clusters. We provide empirical evidence suggesting that the number of empirically meaningful clusters is large in realistic datasets.

% {\color{gray}
% need to directly define cluster
% need to define function class as concatenation of supervised learners
% need to focus more on uniformity
% }


% Why existing theoretical analyses are insufficient: fail to consider inductive bias of model, fail to consider InfoNCE loss

% The inductive bias we consider is a fundamental inductive bias of supervised classifiers - any classifier that classifies points from the same class differently also classifies points from the same class in the training set differently...

% Aligned and and uniform representations on the hypercube are desired because normalized representations (although on the full hypersphere) have been shown to improve training stability and downstream performance compared to Euclidean representations \cite{xu2018spherical,wang2017normface,davidson2018hyperspherical,bojanowski2017unsupervised} and discretization forces clustering. 


% We show that the general class of representations we consider 
% inherits this bias of supervised learning.

% Our work provides a thorough anaylsis of the InfoNCE loss, with contributions summarized as follows.
\begin{itemize} % for any $z \in \mathbb{N}$, 
    \item {\color{red} We show that when the number of clusters $m=2^d$ and the sizes of the clusters are identical, all solutions of the InfoNCE objective optimized over $\mathcal{G}$  are {\em clean} and {\em uniform}, meaning they represent all images from the same cluster identically and  map clusters uniformly on the $d$-hypercube, respectively. 
    {\color{blue} [KS: $d$ is not defined. Further, we consider $d$ boolean functions as making our representation correct ? All that has not been defined in the intro]}
    MARKOV CHAIN
    \item Using these results, we show that  representations on the hypercube learned via the InfoNCE loss optimized over $\mathcal{G}$ yield a single-layer ReLU head that can solve any downstream classification task in which all images in the same cluster have the same label. Conversely, we show that solutions to the InfoNCE loss optimized over an arbitrarily powerful representation class $\mathcal{G}_\star$  cannot have any meaningful downstream performance guarantees on such tasks.
    \item In the agnostic setting with arbitrary numbers and sizes of clusters, we first show that the InfoNCE loss of near-uniform representations is bounded within a short interval around the negative Shannon entropy. Second,  we prove  that representations in $\mathcal{G}$ that are close to uniform under a looser notion of closeness must also be clean if they are minimizers of the InfoNCE  loss on $\mathcal{G}$.  Our sensitivity proof exploits the geometry induced by the inverse maps from the hypercube to the space of images by the pair of representations: the non-clean map, and the perturbed (cleaner) map. These induce a partition over the space of images, leading to multiple cases: in each of the cases, we show that the improvement in the InfoNCE loss due to positive samples outweighs the effects of negative samples while moving from the non-clean to the cleaner representation.
}
    % \item {We show experimentally that the number of clusters is often large thus it makes sense to pack clusters into a hypercube rather  than on the axes.}
\end{itemize}
 \end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[t!]
%\vskip 0.2in
%\begin{center}
% \centerline{\includegraphics[width=0.8\columnwidth]{Spiky1.png}}
%\centerline{\includegraphics[width=0.4\columnwidth]{spikyaugs-3 (6).pdf}}
%\caption{We consider a class of representations consisting of concatenated binary classifiers, with the classification boundaries of two example classifiers shown above ($f_1$ and $f_2$). The classifiers have limited complexity, which induces a clustering of images and their augmentations. Specifically, clusters are sets of images such that are not split by any classifier that does not pass through any augmentation set. In other words, if a classifier intersects a cluster, then it must also intersect at least one augmentation set, e.g. as $f_2$ intersects the blue and green augmentation sets in the Dogs cluster. Our motivating assumption is that the clusters induced by the function class are related to downstream tasks. Images are taken from the Animals V2 dataset \citep{deepnets_2022}.}
%\label{fig:spiky}
%\end{center}
%\vskip -0.2in
%\end{figure}


% \begin{figure}
% \floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,top},capbesidewidth=4cm}}]{figure}[\FBwidth]
% {\caption{We consider a class of representations consisting of concatenated binary classifiers, with the classification boundaries of two example classifiers shown above ($f_1$ and $f_2$). The classifiers have limited complexity, which induces a clustering of images and their augmentations. Specifically, clusters are sets of images such that are not split by any classifier that does not pass through any augmentation set. 
% In other words, if a classifier intersects a cluster, then it must also intersect at least one augmentation set, e.g. as $f_2$ intersects the blue and green augmentation sets in the Dogs cluster. Our motivating assumption is that the clusters induced by the function class are related to downstream tasks.
% Images are taken from the Animals V2 dataset \citep{deepnets_2022}.}\label{fig:spiky}}
% {\includegraphics[width=5cm]{spikyaugs-3 (6).pdf}}
% \end{figure}



\begin{comment}
\begin{SCfigure}[0.5][h]
\includegraphics[width=2.2in]{spikyaugs-3 (6).pdf}
\caption{We consider a class of representations consisting of concatenated binary classifiers, with the classification boundaries of two example classifiers shown above ($f_1$ and $f_2$). The classifiers have limited complexity, which induces a clustering of images and their augmentations. Specifically, clusters are sets of images such that are not split by any classifier that does not pass through any augmentation set. Thus, if a classifier intersects a cluster, then it must also intersect at least one augmentation set, e.g. as $f_2$ intersects the blue and green augmentation sets in the Dogs cluster. Our motivating assumption is that the clusters induced by the function class are related to downstream tasks. Images are from the Animals V2 dataset \citep{deepnets_2022}.\label{fig:spiky}}
\end{SCfigure}
\end{comment}





% \textbf{Notations.}  We use $\mathcal{H}_d$ to denote the $d$-dimensional hypercube and $0_d$ the $d$-dimensional vector of zeros. 
% For a dataset $\mathcal{D}$, we use $x \sim \mathcal{D}$ to denote a random sample drawn uniformly from $\mathcal{D}$.
% % We use $\text{Unif}(\mathcal{D})$ to denote the uniform distribution over the set $\mathcal{D}$. 
% Matrices are denoted in boldface and vectors and scalars in regular type face. 

%,wu2018unsupervised




==> Spiky Augmentations/RelatedWorks.tex <==
\subsection{Related Work}


% \textbf{Understanding contrastive learning.} 
% Contrastive learning encompasses a large class of self-supervised methods that aim to learn expressive representations by maximizing similarity between different views of the same data point and minimizing the average similarity between all pairs of points \cite{wei2021pretrained}. The vast majority of these works optimize InfoNCE-based losses \cite{gutmann2010noise,oord2018representation}, including the widely popular SimCLR framework \cite{chen2020simple}.
% , which differs from the InfoNCE only in its sampling method for negative samples, and in its lack of inclusion of the positive similarity in the uniformity loss.
Several works have aimed to explain the success of contrastive learning in recent years. 
\cite{wang2021understanding} and \cite{wang2020understanding} showed empirically that CL encourages aligned and uniform representations, and improving alignment and uniformity improves downstream performance. The work by \citet{chen2021intriguing} generalizes the InfoNCE loss to a larger family of losses with alignment and uniformity terms weighted according to a hyperparameter. %and shows downstream performancecan be improved by upweighting the positive loss representations and \cite{chen2021intriguing}. % and theoretical approaches. %, our understanding
%grasp of its behavior 
Early theoretical studies attributed the success of CL to its proclivity to maximize the mutual information between augmentations of the same image \citep{bachman2019learning}, but later work cast doubt on this viewpoint by showing that optimizing a tighter bound on the mutual information leads to worse performance \citep{mcallester2020formal,tschannen2019mutual}.
% Many works have studied CL from a theoretical perspective in recent years \cite{tosh2021contrastive,tosh2021contrastivee,wang2020understanding,zimmermann2021contrastive,wen2021toward,chen2021intriguing,haochen2021provable,saunshi2022understanding}, among which a popular approach has been 
% \cite{arora2019theoretical} tried to explain the success of CL by its ability to recover latent variables, but their analysis suggests an upper bound on the number of negative samples which does not hold in practice \cite{nozawa2021understanding}. 
% \citet{tosh2021contrastive} and \citet{tosh2021contrastivee} theorized that conditional independence and redundancy can explain the success of CL with one negative sample per batch.
\citet{wang2020understanding} further {showed} that solutions to the InfoNCE loss are aligned and uniform in the limit of infinite negative samples per batch.

% whereas follow-up work suggests that many negative samples can degrade performance \citep{ash2021investigating,nozawa2021understanding}. 

% However, nearly all of the theoretical analyses in the works assume an unrestricted representation function class and/or infinite negative samples per batch, and/or do not involve the InfoNCE loss. 
% However, the majority of these works consider arbitrary function classes. 
% Other theoretical works that do not assume an unbounded function class include \cite{wen2021toward,tian2022deep}, which studied the feature learning process of CL with shallow neural networks.

% todo: detail ash and nozawa
% \cite{nozawa2021understanding} theory suggesting that the number of negative samples should exceed the number of classes, confirmed by experiments.
% experimental works that show this: - 
% 
% related: On the Surrogate Gap between Contrastive and Supervised Losses
% more recent nozawa paper
% more negative samples always helps 
% theory and experiments rely on pos samples with no augs - unrealistic
% relationship between contrastive and supervised losses

% awasthi paper: conditional independence assumption
% 


%Dual Temperature Helps Contrastive Learning Without Many Negative Samples:
% Towards Understanding and Simplifying MoCo
%  - moco requires huge number of negative samples

% \cite{ash2021investigating} theory suggesting that the number of negative samples should scale with the number of clusters. did not consider temperature (set equal to 1). made conditional independence assumption
% that often does not hold (chaos paper)
% no clusters or other latent variables


%talk about zimmerman and recovering latent variables, cite huang and tsai papers
% \cite{chen2021intriguing} generalizes the InfoNCE loss to a larger family of losses with alignment and uniformity terms weighted according to a hyperparameter and shows downstream performancecan be improved by upweighting the positive loss
% wang paperalignment and uniformity,.. but they show that larger beta should make less clean
% one sentence about empirical works showing that ...
% detail suvrit paper
% note: with particular data generative models\cite{wei2020theoretical} makes impractical expansion assumption. aslo i think tian relu paper assumes overlapping augs?

% li et al 2021: 

% \citep{awasthi2022more} and \citep{bao2022surrogate} show that more negative samples per batch improve downstream performance if the positive pairs are sampled from the underlying clusters rather than from augmentations. both make conditional independence assumption
% effectively these are assuming that the augmentation sets overlap

% \citep{awasthi2022more,bao2022surrogate,ash2021investigating,nozawa2021understanding} study role of the number of negative samples

% \citep{pokle2022contrasting} studied contrastive learning without negative pairs
%\citep{chuang} debiased

% \cite{ji2021power} power of contrast for feature learning, linear case

%multi-sample estimators (van den Oord et al., 2018;
% Poole et al., 2019; Song & Ermon, 2020) popularly used in
% mutual information estimation are substantially related to
% the contrastive loss

% papers that make conditional indepence assumption:
% arora et al. 2019, Lee et al., 2020; Tosh et al., 2021; Tsai et al.,2020). awasthi, bao

% \citep{graf2021dissecting} showed that  (left tab)
% \citep{tsai2020self} 
% \cite{huang2021towards} 
%  

% # awasthi: more negative samples always help


A variety of works have studied CL's ability to recover meaningful clusters or latent variables in the data \citep{arora2019theoretical,tosh2021contrastive,zimmermann2021contrastive,ash2021investigating,nozawa2021understanding,haochen2021provable,shen2022connect,haochen2022beyond,haochen2022theoretical,wang2022chaos,awasthi2022more,bao2022surrogate}. However, the majority of these works consider arbitrary function classes, which requires  strong assumptions on the connectedness of augmentation sets within each cluster, such as assuming positive pairs are conditionally independent given their cluster identity, in order to give downstream guarantees \citep{saunshi2022understanding}.
The work by \citet{haochen2022theoretical} is the most related work to ours, as they study function classes that induce a similar bias towards preserving clusters as ours without any assumption on the connectedness of augmentation sets. 
%
%
%
%
However, their study is focused on 
minimizing a spectral contrastive loss which serves as a surrogate for the more practically used InfoNCE loss. While studying spectral contrastive loss is enlightening and provides some intuition, it cannot be extended to the InfoNCE loss because of two major reasons: % {\color{green} First, the }
{\color{black} First, the loss function fails to highlight the role of finite batches of negative samples, which is a well-studied and key component of the InfoNCE loss \citep{awasthi2022more,bao2022surrogate,ash2021investigating,nozawa2021understanding}.  Second, their analysis does not translate to our setting because the key difficulty in our proof is to show that negative samples promote uniformity; this aspect directly follows with the spectral loss due to the covariance regularizer.}




%% , which is not used in practice .... For example, the spectral loss does not involve finite batches of negative samples, which substantially complicates the analysis of the InfoNCE loss.

% \citet{ash2021investigating} and \citet{nozawa2021understanding} studied the role of the number of  negative samples in CL.



% \cite{nozawa2021understanding} theory suggesting that the number of negative samples should exceed the number of classes, confirmed by experiments.
% \cite{ash2021investigating} theory suggesting that the number of negative samples should scale with the number of clusters. NCE loss, simpler than InfoNCE loss
% \cite{tosh2021contrastivee} 
% \cite{tosh2021contrastive} one negative sample, infoNCE, bounded function classes

% \cite{ji2021power,saunshi2021,tian2022deep} linear case

% \cite{tian2022understanding} nonlinear 

% \cite{jing2021understanding} dimensional collapse. all experiments.
 
 % \citet{wang2020understanding} show that solutions to the InfoNCE loss are uniform and perfectly aligned (represent all positive pairs alike), however this result is limited to the limit as $\ell \rightarrow \infty$. 

% Other works have studied CL's connection with spectral methods \cite{balestriero2022contrastive,haochen2021provable,haochen2022theoretical}. 

% Early interpretations attributed the success of CL to its tendency to maximize the mutual information between augmentations of the same image \cite{}, but optimizing a tighter bound on the mutual information leads to worse performance \cite{}, discrediting this viewpoint. \cite{arora2019theoretical} tried to explain the success of CL by its ability to recover latent variables, but their analysis suggests an upper bound on the number of negative samples which does not hold in practice \cite{}. \cite{zimmermann2021contrastive} shows that solutions to the InfoNCE loss recover latent variables under a generic generative model in the limit of infinite negative samples. 

% Papers showing the effectiveness of pre-trained representations for downstream tasks: \cite{wei2021pretrained} (language models), 
% \cite{mcallester2020formal,tschannen2019mutual}

Additional theoretical works have studied the feature learning process of CL with (stochastic) gradient descent on linear \citep{tian2022deep,ji2021power} and two-layer ReLU neural networks \citep{wen2021toward,tian2022understanding}, properties augmentations must satisfy in order for CL to be successful \citep{tian2020makes}, the role of the projection head in CL \citep{wen2022mechanism,gupta2022understanding}, and the behavior of contrastive losses in (semi-)supervised settings \citep{khosla2020supervised,zheng2021weakly,chen2022perfectly}. Several other works analyze non-contrastive self-supervised learning methods \citep{wei2020theoretical,balestriero2022contrastive,garrido2022duality,lee2021predicting}.
% \cite{tian2020makes} augmentations should preserve task relevant information while decreasing mutual information otherwise
% Lastly, multiple works have studied desirable properties of representations for downstream performance \cite{saunshi2020mathematical,wang2020understanding}. \citet{wang2020understanding}  show empirically that representation uniformity and alignment improve performance on downstream tasks.

% {\color{red} discussion of empirical works that have shown the properties we show}

% \cite{von2021self} showed that maximizing entropy (solving infonce in the limit of infinite negative samples) can separate content vars from style vars under some generative model

% \cite{tian2021understanding} 

% \cite{garrido2022duality} points out the duality between contrastive and non-contrastive methods, \cite{wen2022mechanism} studies the role of the prediction head, \cite{caron2020unsupervised} contrastive clustering

% \cite{wei2021pretrained} pre-training can learn HMM for language that enables solving downstream tasks with simple head. Not contrastive. Does not consider function class bias in pre-training

% \cite{wang2021understanding} increasing $\beta$ leads to more uniformity, decreasing it leads to more alignment.

% nonlinear independent component analysis

% \cite{haochen2021provable} show the equivalence of contrastive learning with the spectral contrastive loss and spectral clustering on a certain graph on the set of images, and show generalization guarantees derived from spectral methods
% shows that contrastive learning with the spectral contrastive loss reduces to spectral clustering on pos pair graph

% \textbf{Comparison with \citet{haochen2022theoretical}.} 
% , in  which the function class' inductive bias is again the inability to represent points from the same cluster differently while also representing points from the same augmentation sets within that cluster similarly. 

% \textit{effect of finitely many negative samples avoided in HaoChen?}
% Second, for fixed representation dimension $d$, \citet{haochen2022theoretical} shows that the CL representation can express $d$ clusters, and allows all possible downstream classification tasks on these $d$ to be clusters to be solved by learning a linear head. In contrast, we show that the CL representation can express $2^d$ clusters, and implement all single-cluster classification tasks by learning a linear head. We can express exponentially more clusters by fitting them on vertices of the hypercube rather than orthogonal coordinate axes as in \cite{haochen2022theoretical}. The trade-off is that since our representations of different clusters are not orthogonal, we cannot express arbitrary labelings. However, we can  lift our representation to $\mathbb{R}^{2^d}$ with a simple, fixed mapping, such that linear functions of the lifted representation can express all labelings of the $2^d$ corresponding to all possible downstream classification tasks. Note their linear example, they can handle $d$ orthogonal tasks with linear head, as can we. There are $2^d$ clusters in their graph, but  it is unclear whether they can implement all $2^{2^d}$ tasks with a single ReLU layer as we can

% We do not assume that the function class does not contain representations that split clusters, which is unrealistic... Rather, we show that these representations are not chosen by InfoNCE due to the spikiness of the augmentation sets with respect to the function class... no 
% their assumption 3.3 is essentially our assumption, except it is an assumption on G, whereas we are only making a coordinate-wise assumption. We need to show the benefit of coordinate-wise representation...

% each coordinate is .... 
% coordinate-wise assumption implies representation-wise assumption, but the inverse isn't true

% They require that $d = m$, where we need only $d=\log(m)$, where $m$ is the number of clusters.

% How many downstream tasks can we implement? With linear head, only $O(d)$ tasks, which is the same as what they get, so what is the point of realizing $2^d$ clusters? When  the head is an MLP with first layer ReLU with $2^d$ neurons, and second and final layer linear, we can implement any function from $\mathcal{H}_d \rightarrow [r]$, which is also effectively what they get. But, they assume $m=r$ (number of labels equals number of clusters). We can get something with the number of clusters way larger than the  number of labels.

% their proof for section 3 is very simple. They show that the optimal representation is a rotation of the coordinate axes. 

% Really we are mapping to the axes in R^(2^d), meaning rep dim is again number of clusters

% can we show that if there are only d clusters, mapping to the axes does not optimize InfoNCE? no, it does optimize it

% \textbf{Representations on the hypercube.}






==> Spiky Augmentations/Theory.tex <==
\section{Bounded Function Class}



% Let $m$ be the number of clusters in the dataset and denote the clusters $S_1,\dots,S_m$.
% Next we formally  define two key notions used throughout the paper. A \textit{uniform} representation is such that the push-forward measure onto the hypercube is uniform, while a \textit{clean} representation is such that every coordinate of the representation is a classifier that respects the equivalence relation between images.
% \begin{definition}[Uniformity]
% A representation $g\in \mathcal{G}$ is {\em uniform} iff $\Pr_{x\sim \I}(g(x)=v)=2^{-d}$ for all $v\in \mathcal{H}_d$.
% \end{definition}
% \begin{definition}[Clean]
% A representation $g\in \mathcal{G}$ is {\em clean} iff $g(x) = g(x')$ for all $x\sim x'$. A classifier $f\in \F$ is {\em clean} iff $f(x) = f(x')$ for all $x\sim x'$.
% \end{definition}
% \begin{assumption}[Realizability]\label{assump:realizability}
%     There exists a $g \in \mathcal{G}$ that is both clean and uniform.
% \end{assumption}

% \begin{assumption}[old] \label{assump:spiky-full}
% For any $f\in \mathcal{F}$ and any cluster $C$, let $p(f,C)\coloneqq \min(1-\mathbb{P}_{x_1^- \sim C}[f(x)=1],\mathbb{P}_{x_1^- \sim C}[f(x)=1])$ and $e(f,C)\coloneqq \mathbb{P}_{x \sim \bar{C}, x^+ \sim \mathcal{A}(x)}[f(x)\neq f(x^+)]$. Then for some $\delta\in (0,1]$, a dataset is called $\delta$-spiky with respect to the function class $\mathcal{F}$ if
% \begin{align}
%     \delta p(f,C) \leq e(f,C) \leq 2 p(f,C)
% \end{align}
% for all $f\in \mathcal{F}, C$.
% \end{assumption}

% \begin{assumption}[Regularity of $\mathcal{F}$ w.r.t. augmentations] \label{assump:spiky}
% For any $f\in \mathcal{F}$, for all clusters $j\in [m]$, if $f(x)\neq f(x')$ for some $x\sim x'$, then $\exists A, A'\in \A$, $x\in \I$ such that $f(A(x))\neq f(x)$.
% \end{assumption}

% \subsection{Finite batch size}
% Much of the difficulty in the analysis of the InfoNCE loss comes from the fact that the negative term in the loss is a finite sample sum rather than an expectation. The case $\ell \to \infty$ has been considered before; we will derive some properties for our specific setting where the representations are constrained to the Boolean hypercube.
% \begin{lemma}

% \end{lemma}

\input{Theory/Bias.tex}
\input{Theory/Realizable.tex}
\input{Theory/Downstream.tex}
\input{Theory/Agnostic.tex}
\input{Theory/UniformityProofSketch.tex}
% \input{Theory/SparseCoding.tex}

==> Spiky Augmentations/Theory/Agnostic.tex <==

\section{Results for the Agnostic Setting}\label{section:agnostic}


% under a natural  assumption on the function class, InfoNCE still learns clean representations that maximize a quantity closely related to entropy over the feature space.

\begin{comment}


Recall that $\mathcal{D}_g$ is the distribution over the hypercube induced by the representation $g$ and the set of images $D_\circ$. The {\em Shannon entropy} of $\mathcal{D}_g$ is defined as:
\begin{align}
    H(\mathcal{D}_g) \coloneqq -\sum_{v \in \mathcal{H}_d} \mathcal{D}_g(v)\log(\mathcal{D}_g(v))
\end{align}
% , where there does not exist a clean, uniform representation. While we conjecture that our results hold in general, we can prove our result only when $d=1$ and  $l=1$.
% \begin{conjecture}[Informal] The minimizer of Equation \ref{eq:InfoNCE} is a clean representation $g$ that maximizes the uniformity of $g$ over clean representations.
% \end{conjecture}
% While the correct notion of maximizing the uniformity of normalized representations in the finite sample agnostic case unclear, it is natural to suppose it is related to entropy. Note that the connection between the negative term in the InfoNCE loss and entropy has been discussed before, we restate it here for completion and because we would like to apply specifically to our setting on the hypercube.
Next we show that the loss $\tilde{\mathcal{L}}$ in Equation \ref{eq:uniformity} behaves like the Shannon entropy near uniform representations. 

\begin{lemma}\label{lemma:entropy}  Consider a representation $g$ such that $\mathcal{D}_g$ satisfies $c_12^{-d}\le \mathcal{D}_g(v)\le c_2 2^{-d}$ for constants $c_1,c_2$  for every $v\in \uH^d$, and suppose $\beta \geq \frac{\log(d)+ 1}{2}$ and $\ell > \frac{d\log\frac{1}{\delta}}{c_1 \epsilon^2} 2^d$ for any $\epsilon\in (0,1)$.
% We have
% $e^{-2\beta}d\le \frac{1}{2}$. 
Then for $\hat{\mathcal{L}}(\mathcal{D}_g)$ defined in \ref{eq:uniformity}, 
\begin{align}
% -H(\mathcal{D}_g)-\epsilon &\le \tilde{L}(\mathcal{D}_g) - \log l - \beta d \le -H(\mathcal{D}_g) + (1-\delta)\left(\epsilon + \frac{2de^{-2\beta}}{c l}\right)+\delta(\log l + \beta d) 
-H(\mathcal{D}_g)-\epsilon  &\le \hat{\mathcal{L}}(\mathcal{D}_g) - \log \ell - \beta d \nonumber \\
\hat{\mathcal{L}}(\mathcal{D}_g) - \log \ell - \beta d &\le -H(\mathcal{D}_g) + (1-\delta)\left(\epsilon + \frac{2c_2 de^{-2\beta}}{c_1 \ell}\right) +\delta(\log \ell + \beta d)  \nonumber 
\end{align}
{\color{red}Furthermore, for any $g$ , we have 
% \begin{equation*}
% -H(\mathcal{D}_g) - \epsilon - c\log c - dc\le \tilde{L}(\mathcal{D}_g) - \log \ell - \beta d
% \end{equation*}
\begin{equation*}
-H(\mathcal{D}_g) - \epsilon - c\log c - dc\le \tilde{L}(\mathcal{D}_g) - \log \ell - \beta d
\end{equation*}
}
\end{lemma}
% Lemma \ref{lemma:entropy} shows that 
% A  proof of the above lemma is provided in Appendix \ref{appendix:uniformity}. 
It is well-known that the uniform distribution maximizes the Shannon entropy, so Lemma \ref{lemma:entropy} suggests that the InfoNCE loss encourages uniform representations. {\color{red} While previous results have drawn connections between the entropy and InfoNCE loss, ours is the first to formalize this connection with finite negative samples \citep{}.}


 {\color{black}
% Further recall that $\Gamma_{\mathbf{c}}$ denotes the cluster of images with content $\mathbf{c}$, $\Gamma_{\mathbf{c},\circ}$ denotes the set of natural images in that cluster, and 
% Recall that for a set of images $B\subseteq D$,  $\|B\|_\circ \coloneqq \mathbb{P}_{x \sim D_{\circ}}(x \in B)$ and $\|B\| \coloneqq \mathbb{P}_{x \sim D}(x \in B)$.}

%{\color{red} ... what is part B saying?}

\end{comment}

In this section, we consider the setting in which there may not exist any cluster-preserving and uniform representation (that is, Assumption \ref{assump:realizability} is violated). We show that even in this setting, the InfoNCE loss prioritizes cluster-preserving representations. Specifically, we show that if an optimal solution of the InfoNCE loss on $\mathcal{G}$ is close to uniform, then it must also be cluster-preserving. This result requires two new assumptions that we describe below. 

First, the function class  $\mathcal{F}$ must be closed under operations that make classifiers cluster-preserving, in the sense that if $f\in \mathcal{F}$ and $f$ does not preserve the cluster $\Gamma_{\mathbf{c}}$, then the two perturbations of $f$ that preserve $\Gamma_{\mathbf{c}}$ (by assigning $\pm 1 $ to all images within it) and do not change $f$ otherwise are also in $\mathcal{F}$.
\begin{assumption}[Expressivity of $\mathcal{F}$]\label{assump:exist}
For any cluster $\Gamma_{\mathbf{c}}$, if any $f\in \mathcal{F}$ is such that $f(x)\neq f(x')$ for some $x,x'\in \Gamma_{\mathbf{c}}$, then $f' \in \mathcal{F}$ and $f'' \in \mathcal{F}$, where $f'(x) = f''(x) = f(x) \;  \forall x \notin \Gamma_{\mathbf{c}}$, and $f'(x)=1, f''(x)=-1 \;\forall x \in \Gamma_{\mathbf{c}}$.
\end{assumption}

% \begin{assumption}[$(\gamma, \delta)$-Regularity of $\mathcal{F}$] \label{assump:spiky_complete}
% A function class $\F$ is called $(\gamma, \delta)-$regular if 
% \begin{enumerate}[ref={\theassumption.\Alph*}]
% \item \label{assump-a}For every $f\in F$, for any $x\in D_\circ$, $$\Pr_{x^+\sim \text{Unif}( \kappa(x))}[f(x)\ne f(x^+)] \le \gamma.$$
% \item \label{assump-b}For any $f\in \F\setminus \F_c$, let 
% $$\Delta_f := \min_{f_c\in \F_c} \Vert \{x \in D_\circ \mid f(x) \ne f_c(x)\}\Vert_\circ.$$ 
% Then we have $\Pr_{x^+\sim \text{Unif}( \kappa(x))}[f(x)\ne f(x^+)] \ge \delta \Delta_f$.
% \end{enumerate}
% \end{assumption}
Next we define a regularity condition of a function class and augmentation set that
captures the extent to which non-cluster-preserving classifiers classify  images in positive pairs differently within clusters that they intersect. 
% Recall that  a cluster is a set of points classified alike by all   classifiers that classify the samples in every positive pair alike. 
% This means that any classifier that splits a cluster (i.e., any non-clean classifier) must also split an augmentation set within that cluster, as we used critically in the proof of Theorem \ref{thm:uniformandclean}. 
So far, we have only assumed that non-cluster-preserving classifiers misclassify at least  
% does not entail that non-clean classifiers must in 
% only implies that any non-clean classifier classifies the samples in at least 
{\em one}  positive pair differently within any cluster they intersect (Assumption \ref{assump:spikyaug}).
However, for regular classes of binary classifiers and intertwined augmentation sets within clusters, we can expect that the number of positive pairs split in a cluster that are split by any binary classifier scales with the number of negative pairs in the same cluster that are split by the classifier.
% Here, we define the regularity of a class of binary classifiers  by the minimum number of positive pairs in a cluster that must be misclassified by any classifier in the class that does not preserve that cluster. 
% Recall that Theorem \ref{thm:uniformandclean} only required 
For a set of images $B\subseteq D$, we employ the notations  $\|B\|_\circ \coloneqq \mathbb{P}_{x \sim D_{\circ}}[x \in B]$ and $\|B\| \coloneqq \mathbb{P}_{x \sim D\setminus D_\circ}[x \in B]$.
% Further, recall that $\Gamma_{\mathbf{c},\circ}\coloneqq {\Gamma}_{\mathbf{c}}\cap D_\circ$.
\begin{definition}[$\delta$-Regularity] \label{defn:reg} %\label{assump:spiky_complete}
% A function class $\F$ is called $(\gamma, \delta)-$regular if 
% \begin{enumerate}[ref={\theassumption.\Alph*}]
% \item \label{assump-a}For every $f\in F$, for any $x\in D_\circ$, $$\Pr_{x^+\sim  \kappa(x)}[f(x)\ne f(x^+)] \le \gamma.$$
% \item \label{assump-b}
For any $f\in \F$, let $\Sigma_f \coloneqq \{\mathbf{c}\in {C}: %\; \text{s.t.}\; 
\exists  x,x'\in \Gamma_{\mathbf{c}} \; \text{s.t.}\; f(x) \neq f(x')\}$ be the set of content variables corresponding to clusters split by $f$. 
% {\color{blue} Let $S_{\mathbf{c},\circ}$ be ...}
For all ${\mathbf{c}} \in \Sigma_f$ and $\sigma \in \{-1,1\}$, define %\begin{align}
    $f^{({\mathbf{c}},\sigma)}(x) \coloneqq \begin{cases} f(x) & x \notin \Gamma_{\mathbf{c}} \\
    \sigma & x \in \Gamma_{\mathbf{c}} \\
    \end{cases}$ as the classifier that outputs the same label as $f$ on all images not in $\Gamma_{\mathbf{c}}$ and  $\sigma$ on $\Gamma_{\mathbf{c}}$. Further define 
    %,\quad  \nonumber \\
    $\Delta_{f,\mathbf{c}} \coloneqq  %\min_{{\mathbf{c}}  \in \Sigma_f} 
    \min_{\sigma \in \{-1,1\}} \Vert \{x \in \Gamma_{\mathbf{c},\circ} \mid f(x) \ne f^{({\mathbf{c}},\sigma)} (x)\}\Vert_\circ $ as the minimum measure of the set on which $f^{\mathbf{c},\sigma}$ and $f$ differ among all possible choices of $\sigma \in \{-1,1\}$. 
%\end{align}
% Lastly, let $R\coloneqq \{x^+\in A(x): x\in \Gamma_{\mathbf{c},\circ}, \; f(x)\ne f(x^+)\}$ be the set of   augmentations in the cluster $\Gamma_{\mathbf{c}}$ that are misclassified by $f$.
Then $(\F,\Lambda)$ is $\delta-$regular if for all $\mathbf{c} \in \Sigma_f$,  $\|\{\mathcal{A}(x):\mathcal{A}\in \Lambda, x\in \Gamma_{\mathbf{c},\circ}, \; f(x)\ne f(x^+)\}\| \ge \delta \Delta_{f,\mathbf{c}}$.
% \end{enumerate}
\end{definition}

 % Assumption \ref{assump-a} states that \textit{every} classifier in the function class $\F$ can only separate an image from some $\gamma$ fraction of its augmentations. Suppose the natural images are points in $\R^D$, and suppose an augmentation was a perturbation of the natural image by a mean-zero Gaussian. If the class $\F$ consisted of linear half-spaces, then this assumption is satisfied with $\gamma = \frac{1}{2}$ (any halfspace that contains the center of the Gaussian must contain at least half of the augmented data).

 % Below, we effectively assume that any non-clean classifier that splits $k$ natural images from the rest of their cluster must also split a constant fraction of $k$ augmentations from their natural images in that cluster.

\noindent Definition \ref{defn:reg} states that a function class and set of augmentations $(\mathcal{F},\Lambda)$ is $\delta$-regular if the number of positive pairs split by a classifier that intersects a cluster is at least $\delta$ fraction of the extent to which the classifier intersects the cluster. If classifier $f\in \mathcal{F}$ barely intersects the cluster, i.e., classifies most natural images from the cluster alike, then $\Delta_{f,\mathbf{c}}$ is small and the lower bound on the number of positive pairs that it intersects is weaker. However, if $f$ splits the cluster almost in half, then $\Delta_{f,\mathbf{c}}$ is large and the classifier separates many augmentations from their associated natural images within the cluster.  
Next, we state our regularity assumption and the result for the agnostic case. 
% This notion of regularity is qualitatively equivalent to the one assumed by \cite{haochen2022theoretical} in their Assumption 3.3. %Next we assume that $(\mathcal{F},\Lambda)$ is indeed 0.6-regular.
% This definition formalizes the intuition that for any reasonably restricted class of classifiers $\mathcal{F}$ and intertwined augmentations $\Gamma$, the augmentation sets are sufficiently dense within clusters and non-smooth  relative to the functions in the class, such that any classifier that separates augmentation sets from related images must also separate a commensurate number of augmentations from their natural images.
% For our main result, we require that $\F$ is at least $0.6-$regular.

% , and is in the same spirit as Assumption 3.3 in \citep{haochen2022theoretical}

% $\Delta_{f,\mathbf{c}}$ is the smallest change that can be incurred in $f$ by making it clean with respect to any of the clusters that it cuts. 

% if the misclassification error on augmented pairs for any  classifier in $\F$ that is not clean with respect to the cluster $\Gamma_{\mathbf{c}}$ is lower bounded at least a $\delta$-fraction of

% the number of natural images that the closest classifier that is clean with .



% In particular, let $\Sigma_f$ be the set of cluster indices corresponding to clusters cut by $f$. 



% The assumption is that among the intersected clusters, the probability that   is at least a $\delta$-fraction of $\Delta_{f,\mathbf{c}}$. Such an assumption is natural, as it essentially says that any classifier that cuts a cluster must also cut augmentation sets within that cluster to a commensurate extent, and holds as long as the clusters are sufficiently dense and non-smooth relative to $\mathcal{F}$.}
% misclassifies some natural images
% (defined as being those it disagrees with  $f$ on, where $f$ is its closest neighbour in $\F_c$),
% then there is a lower bound on its supervised error on the task $f$. %{\color{red} why?}


% \begin{theorem}\label{thm:agnostic}
% Consider the InfoNCE objective (\ref{eq:InfoNCE}) when $l\ge d^{\frac{3}{2}}2^d \frac{\log 1/\delta}{\epsilon^2}$, and suppose $\beta > 10\log l$. Under Assumptions \ref{assump-a} and \ref{assump-b}, the optimal representation is clean and such that it maximizes the entropy of the downstream representations to within $o(d)$.
% \end{theorem}


% if none of the inverse sets are negligible, then Bv negligible implies Av cap C  is non-negligible, so we are fine.

% if some of the inverse sets are negligible, then Bv might be negligible. use epsilon to account for this. Also, some Av might be in the bad range, but they must also be in C, so we're fine.

% the bad case is if Bv is negligible and Av is negligible. But can we account for this? no it doesn't help. Note that even if Bv is negligible, there can be a large Av' that encompasses the same augmentation set

% if we say the inverse sets are either zero or larger than the bad range, then we don't need the epsilon.

\begin{assumption}[$\delta$-Regularity of $(\mathcal{F},\Lambda)$] \label{assump-b}
    The pair $(\mathcal{F},\Lambda)$ is $\delta-$regular with $\delta\geq 0.4$.
\end{assumption}

\vspace{-1mm}
% Now we are ready to state our main result for the agnostic setting. The below theorem states that if $g$ is in some sense close to a uniform representation, it must be clean in order to optimize the InfoNCE loss with sufficiently large $\ell$ and $\beta$. 

%Our main result for the agnostic setting states that if $g$ is in some sense close to a uniform representation, it must be cluster-preserving in order to optimize the InfoNCE loss. % with sufficiently large $\ell$ and $\beta$. 

 % \vspace{-10mm}

\vspace{-1mm}
\begin{theorem} \label{thm:agnostic}
% Let $\ell = \frac{C}{\epsilon} d 2^d $ for an absolute constant $C$ and $\beta \geq c_3 2^d$. 
Suppose Assumptions \ref{assump:exist} and \ref{assump-b} hold and $g= [f_1,...,f_d]$ is \textbf{not} cluster-preserving with 
$\min_{j\in [d]} \min_{\mathbf{c} \in \Sigma_{f_j}} \mathbb{P}_{x,x'\sim D}[x, x' \in \Gamma_{\mathbf{c}},f_j(x)\neq f_j(x')] \geq \epsilon >0$. Let $\ell \geq \frac{ c  }{\epsilon} d 2^d $, $\beta \geq {c}\log(\frac{c}{\epsilon}) 2^d$ for a sufficiently large constant $c$.
% $\min_{j\in [d]} \min_{\mathbf{c} \in \Sigma_{f_j}} \|\{x^+\in A(x): x\in \Gamma_{\mathbf{c},\circ}, \; f_j(x)\ne f_j(x^+)\}\| \geq \epsilon >0$. 
Moreover, suppose $g$
 is close to a uniform
representation in the sense that\footnote{Note that this near-uniformity condition allows for representations that for each vertex put  mass at least a constant factor of $\frac{1}{d}$ times $2^{-d}$, or essentially treat the vertex as   inactive,
 % Recall that for a uniform representation, $\mathcal{D}_g(v) = 2^{-d}$ for all $v$. Here, we consider representations that for all vertices have a least a factor of $\frac{\log(d)}{d}$ from $2^{-d}$ mass, or treat the vertex as essentially  inactive, 
 which allows for the case wherein the number of clusters is less than $2^d$ and some vertices are inactive for cluster-preserving representations.}  $\mathbb{P}_{x\sim D_\circ}[g(x)=v] \geq \frac{10}{ c d2^d}$ 
or $\mathbb{P}_{x\sim D_\circ}[g(x)=v]  \leq \frac{ \epsilon}{ 100 c d 2^{2d}} $
% $\|Q_v\|_\circ > \frac{\log(\eta)}{c 2^d}$ or $\|Q_v\|_\circ \leq \frac{c'}{ \eta d 2^{2d}}$ 
for all $v\in \mathcal{H}_d$.
Then $g$ is \textbf{not} a minimizer of the InfoNCE loss. 
% $\mathcal{L}(g)> \mathcal{L}(g')$ for some nearby representation $g'$. 
% Consider the InfoNCE objective \ref{eq:InfoNCE} when $l \ge m \log m$. 
% The optimal representation is clean and such that it maximizes the entropy of the downstream representations to within an additive error.
\end{theorem}


\begin{comment}

\begin{figure}[t]
\centering
% \resizebox{5cm}{!}{\input{spikyproof.pdf}} %{\input{dirtyToClean.tikz}}
\centerline{\includegraphics[width=0.9\columnwidth]{spikyproof2.pdf}}
\caption{Example partitioning of images with $d=2$ and $D\subset \mathbb{R}^2$. Green triangles denote natural images, and black ellipses their corresponding augmentation sets (we have drawn the augmentation sets as ellipses for ease of presentation, but in reality they are typically highly non-smooth and non-contiguous). Clusters are indicated by dotted black ellipses. Here the ``cleaner'' representation $g'$ is constructed by making $f_1$ clean with respect to the cluster $S_{\mathbf{c}'}$. The region $R$  consisting of augmentations in $S_{\mathbf{c}'}$ misclassified by $f_1$ is shaded red, and the set $B$ of images which are classified differently by $f_1$ and $f_{1}^{(\mathbf{c}',\sigma')}$ is indicated by blue diagonal lines. By Assumption \ref{assump-b}, $\|R\| \geq \delta \|B\|_{\circ}$.} \label{fig:agnostic}
 % Illustration of a perturbation from a representation that is not clean to a cleaner representation. The lines represent the decision boundary of a single coordinate of the representation, which is hypothesized to be non-clean. The black dots represent the natural images that correspond to each of the clusters/augs sets, while the ellipses represent the augmentation sets corresponding to the black dots. The red shaded region represents the misclassification of the classifier corresponding to the non-clean coordinate.
\end{figure}
\end{comment}

%\begin{comment}
\begin{figure}
  \begin{minipage}[c]{0.35\textwidth}
  \vspace{-6mm}
    \includegraphics[height=2.4in,width=1.9in]{spikyproof3.pdf}
  \end{minipage}\hfill %\hspace{-0.5in}
  \begin{minipage}[c]{0.65\textwidth}
\caption{Example partitioning of images with $d=2$ and $D\subset \mathbb{R}^2$. Green triangles denote natural images and solid black ellipses denote their corresponding augmentation sets (here we have drawn the augmentation sets as compact convex sets for ease of presentation, but in reality they may be non-simply connected and non-smooth). Clusters are indicated by dotted black ellipses. The non-cluster-preserving representation $g=(f_1,f_2)$, and we construct $g'=(f_1',f_2)$ by making $f_1$ preserve the cluster $\Gamma_{\mathbf{c}}$. The region $R$  consisting of augmentations in $\Gamma_{\mathbf{c}}$ misclassified by $f_1$ is shaded red, and the set $E$ of images which are classified differently by $f_1$ and $f_{1}'$ is indicated by blue diagonal lines. By Assumption \ref{assump-b}, $\|R\| \geq \delta \|E\|_{\circ}$, where $\|B\| \coloneqq \mathbb{P}_{x \sim D\setminus D_\circ}[x \in B]$  and  $\|B\|_\circ \coloneqq \mathbb{P}_{x \sim D_{\circ}}[x \in B]$ for any set of images $B \subseteq D$ \label{fig:agnostic}.
}
\end{minipage}
\end{figure}
%\end{comment}



  
\begin{proof}[Proof sketch of Theorem \ref{thm:agnostic}] For a non-cluster-preserving representation $g$ that is ``close" to a uniform representation, we construct a nearby representation $g'$ by changing one coordinate of $g$ such that it preserves one additional cluster, and show that the resulting $g'$ achieves smaller InfoNCE loss than $g$. 
% We construct $g'$ by changing only one coordinate of $g$ such that it preserves one cluster that it intersects. 
In particular suppose WLOG that $f_1$ does not preserve the cluster $\Gamma_{\mathbf{c}}$.
% has largest misclassification of positive samples on its most misclassified cluster among all $d$ classifiers in $g$, specifically that $1 \in \arg\max_{j\in [d]} \max_{\mathbf{c}' \in \Sigma_{f_j}} \|\{x^+\in A(x): x\in \Gamma_{\mathbf{c}',\circ}, \; f_j(x)\ne f_j(x^+)\}\|$. 
% meaning Suppose WLOG  that $1 \in \arg\max_{j\in [d]} \max_{\mathbf{c} \in \Sigma_{f_j}} \|\{x^+\in A(x): x\in \Gamma_{\mathbf{c},\circ}, \; f_j(x)\ne f_j(x^+)\}\|$, meaning 
Further, let $f_1^{(\mathbf{c},\sigma)}$ be the smallest perturbation of $f_1$ that preserves $\Gamma_{\mathbf{c}}$, as defined in Definition \ref{defn:reg}.
% $ \sigma \in \arg \min_{\sigma' \in \{-1,1\}} \Vert \{x \in D_\circ \mid f_1(x) \ne f_{1}^{(\mathbf{c},\sigma')} (x)\}\Vert_\circ $, using the notation defined in Assumption \ref{assump-b}, and 
Denote $f_1'= f_1^{(\mathbf{c},\sigma)}$.  {By Assumption \ref{assump:exist}, $f_1' \in \mathcal{F}$.} 
Construct $g' =[f_1',f_2,\dots,f_d] \in \mathcal{G}$. 
Note that $g'$ is equivalent to $g$ on all but one coordinate, and the one differing coordinate differs only on one cluster.

% where 
% \begin{align*}
% \mathcal{L}_{\text{pos}}(g) &:= -\beta \mathbb{E}_{x, x^+}\left[g(x)^\top g(x^+)\right] \nonumber \\
% {L}_{\text{neg}}(g) 
% &:= \mathbb{E}_{x,x^+, \{x^-_i\}_{\ell}} \bigg[\log\bigg({ e^{\beta g(x)^\top g(x^+)}\!+\!\sum_{i=1}^\ell e^{\beta g(x)^\top g(x^-_{i})}  } \bigg)\bigg] \nonumber
% \end{align*}

% To analyze the negative loss, it is helpful to first partition the space 

To characterize the variation in the InfoNCE loss when moving from $g$ to $g'$, we first consider a specific partition of the space of images defined based on the representations $g$ and $g'$. In particular, for a given vertex $v \in \mathcal{H}_d$, consider the set $Q_v := \{x \in {D} : g(x)=v, g'(x)=v \}$ which denotes the set of images that both $g$ and $g'$ map to vertex $v$, and the set $E_v := \{x \in  {D} : g(x)= v, g'(x)\neq v \}$ which denotes the set of images that $g$ maps to $v$ and $g'$ maps to another vertex. Considering these definitions, the set  $Q:= \cup_{v \in \mathcal{H}_d} Q_v$ corresponds to the set of all images that $g$ and $g'$ map to the same vertex, while $E:= \cup_{v \in \mathcal{H}_d} E_v$ denotes the set of all images which $g$ and $g'$ map to different vertices. Based on this construction, it is not hard to observe that for any $v\neq v'$ the sets $Q_v$, $Q_{v'}$, $E_v$, and $E_{v'}$  are disjoint, and each image belongs to either some $Q_v$ or $E_v$. Hence, the concatenation of these sets partitions the space of images. 
 Figure \ref{fig:agnostic} illustrates this partition for a special case with $d=2$. 
 % Finally, note that the sets $Q$ and $E$ are also disjoint and their union is the set of all images. 
 The above partition is critical as we divide our sensitivity analysis into multiple cases based on the location of the positive and negative images in this partition. 



 
% For all $v \in \mathcal{H}_d$, define the sets $Q_v := \{x \in {D} : g(x)=v, g'(x)=v \}$ and $E_v := \{x \in  {D} : g(x)= v, g'(x)\neq v \}$.  

 
%Let  $Q:= \cup_{v \in \mathcal{H}_d} Q_v$ and $E:= \cup_{v \in \mathcal{H}_d} E_v$, meaning $Q$ is the set of images on which $g$ and $g'$ are the same, whereas $E$ is the set of images on which they differ.
% Note that $\|B\|_\circ = \Delta_{f_1} $ (defined in Assumption \ref{assump-b}) by construction of $g'$. 
%Also observe that all of the $Q_v$'s and $E_v$'s are disjoint, and $Q \cup E = {D}$. 

Let us define $\mathcal{L}^+$ and $\mathcal{L}^-$ as the alignment and uniformity losses in \eqref{eq:InfoNCE}, respectively. We refer to $\mathcal{L}^+$ as the positive part of the loss as it deals with positive samples (augmented images), and we  refer to $\mathcal{L}^-$ as the negative part of the loss as it contains negative samples. 
To prove that moving from $g$ to $g'$ decreases the loss, i.e., $\mathcal{L}(g)- \mathcal{L}(g')>0$, we show that the amount that the positive part of the loss decreases is more than the amount the negative part might increase: 
$\mathcal{L}^+(g) - \mathcal{L}^+(g') > \mathcal{L}^-(g') - \mathcal{L}^-(g)$.
To do so, first, note that the variation in the positive part is
\begin{align}
    \mathcal{L}^+(g) - \mathcal{L}^+(g') = 2\beta \left(\Pr\left[x\in Q, x^+\in E\right] + \Pr\left[x\in Q, x^+\in E\right]\right). \label{eq:sumv} % =: \Lambda^+. _{x \sim D_\circ, x^+\sim A(x)}
\end{align}
This holds as $ \beta g(x)^\top g(x^+)=\beta g(x)'^\top g'(x^+)$ except for the cases that $x\in Q, x^+\in E$ or $x\in Q, x^+\in E$. In these two cases, they differ by $2\beta$. Note that the augmentations that belong to either of these two cases lie in the area shaded red in Figure \ref{fig:agnostic}. {{
% Recall $f_1^{(\mathbf{c},\sigma)}(x)$ as the replacement of $f_1$ in the representation $g'$. Now define the set $Z \coloneqq \{ Q_v:f_1^{(\mathbf{c},\sigma)}(x) = f_1(x') \; \forall x \in Q_v, x' \in E\}$ as the set of images that $g$ and $g'$ 
% (e.g. $\{Q_{v_1},Q_{v_2}\}$ in Fig. \ref{fig:agnostic}). 
We refer to the set of augmentations in this region as $R$, in other words, $R$ is the set of augmentations in $\Gamma_{\mathbf{c}}$ that are classified differently than their natural image by $f_1$. 
Thus, we can write $\mathcal{L}^+(g) - \mathcal{L}^+(g') = 2\beta\|R\|$.
% , i.e. the size of $R$ is the error of $f_1$ on the positive loss on  $\Gamma_{\mathbf{c}'}$. 
}}

%Note that the expression  $\Pr\left[x\in Q, x^+\in E\right] + \Pr\left[x\in E, x^+\in Q \right] $ is exactly the measure of the region $R$ shaded red in Figure \ref{fig:agnostic}.









% In particular, we construct $g'$ by making one classifier in $g$ clean with respect to one cluster 
% Denote by $\Vert \cdot \Vert_\circ$ the measure associated with natural images, that is 
% $$ \Vert A\Vert_\circ \coloneqq \Pr_{x\sim \I}[x\in A].$$ Similarly denote by $\Vert \cdot \Vert$ the measure associated with augmentations, so 
% $$ \Vert A\Vert \coloneqq \Pr_{x\sim \I, x^+\sim \A(x)}[x^+\in A].$$


Next, we consider the difference in negative parts of the loss. To bound this difference, we leverage the partitioning of the space of images defined above to 
% consider all disjoint cases with $x \in Q_v$ and $x \in E_v$, for all vertices $v$. We 
decompose the variation of the losses based on the set that image $x$ belongs to. In particular, if we define the function $\mathcal{L}^-_{B}(g):=\mathbb{E}_{x,x^+, \{x^-_i\}_{\ell}} \big[ \chi({B})  \log\big({ e^{\beta g(x)^\top g(x^+)}+\sum_{i=1}^\ell e^{\beta g(x)^\top g(x^-_{i})}  } \big)\big] $ for any event~$B$, where $\chi({B})$ is the indicator random variable for the event $B$, then using the fact that each image $x$ either belongs to one of the $Q_v$'s or $E_v$'s we can write  
\begin{align}
    \mathcal{L}^-(g') - \mathcal{L}^-(g) = \sum_{v \in \mathcal{H}_d} \big[\mathcal{L}^-_{\{x\in Q_v\}}(g') - \mathcal{L}^-_{\{x\in Q_v\}}(g)\big] +\big[\mathcal{L}^-_{\{x\in E_v\}}(g') - \mathcal{L}^{-}_{\{x\in E_v\}}(g)\big],
\end{align}
Since the cases with $x \in E_v$ utilize similar analysis for those with $x \in Q_v$, we focus on the $x \in Q_v$ cases here and defer the $x \in E_v$ cases to Appendix \ref{appendix:agnostic}. 

To analyze $\mathcal{L}^-_{\{x\in Q_v\}}(g') - \mathcal{L}^-_{\{x\in Q_v\}}(g)$, we first observe that this difference is non-positive for a subset of the $Q_v$'s. Note in Fig. \ref{fig:agnostic} that if $x$ belongs to  $Q_{v_1}$ or $Q_{v_2}$, then moving from $f_1$ to $f_1'$  decreases the representation similarity for some pairs of negative samples (those with $x_i^-\in E$) while keeping the rest the same. So, the negative part of the loss cannot increase going from $g$ to $g'$ if $x$ lies  in either $Q_{v_1}$ or $Q_{v_2}$. We formally define this set of $Q_v$'s as $Z \coloneqq \{Q_{v}: f'_{1}(x)\neq f'_1(x^-) \; \forall x \in Q_{v}, x^-\in E\}$.
At a high level, the reason this definition implies the negative part of the loss does not increase if $x \in Q_v \in Z$ is because $f_1$ and $f_1'$ must agree on $Q_v\in Z$  and disagree on $E$, so since $f_1'$ differs on $Q_v\in Z$  and $E$, $f_1$ must agree on these sets. Thus, the similarity between negative pairs consisting of $x \in Q_v \in Z$ and $x_i^-\in E$ diminishes when moving from $g$ to $g'$. Thus, we have  
\begin{align}
   \sum_{v \in \mathcal{H}_d} \mathcal{L}^-_{\{x\in Q_v\}}(g') - \mathcal{L}^-_{\{x\in Q_v\}}(g) \leq \sum_{v \in \mathcal{H}_d} \mathcal{L}^-_{\{x\in Q_v\notin Z\}}(g') - \mathcal{L}^-_{\{x\in Q_v\notin Z\}}(g)  
\end{align}



% We know $f_1(x) = f_1'(x)$ by definition of $Q_v$

% If $x^-\in Q_{v'}$ then $f_1(x^-) = f_1'(x^-)$ by definition of $Q_v'$
% Therefore $g'(x)^\top g'(x^-) = g(x)^\top g(x^-)$ since no other coordinates change

% If $x^-\in E$ then $f_1(x^-) \neq f_1'(x^-)$ by definition of $E$
% Also, $f_1'(x) \neq f_1'(x^-)$  by definition of Z
% Therefore $f_1(x) = f_1(x^-)$
% Therefore $g'(x)^\top g'(x^-) = g(x)^\top g(x^-) - 2 $ since no other coordinates change

% In all cases $g'(x)^\top g'(x^-) \leq g(x)^\top g(x^-)$.


% then $\mathcal{L}^-_{\{x\in Q_v\}}(g') - \mathcal{L}^-_{\{x\in Q_v\}}(g) \leq 0$. This is best understood via  Fig. \ref{fig:agnostic}, in which $Z = \{Q_{v_1},Q_{v_2}\}$. Observe that if $x \in Q_{v_1}$ or $x \in Q_{v_2}$, the representations of all negative samples only become less 






% We first note that  $\mathcal{L}^-_{\{x \in Q_v \in Z\}}(g) - \mathcal{L}^-_{\{x \in Q_v \in Z\}}(g')> 0$ since  $g'(x^-)$ is less similar to $g'(x)$ than $g(x^-)$ is to $g(x)$ for all $x^- \in B$ and $x \in Q_v \in Z$ (as seen in Fig. \ref{fig:agnostic}), and the similarities are unchanged for $x^+$ and all other $x^-$. So, we can upper bound $$\mathcal{L}^-(g') - \mathcal{L}^-(g) \leq \sum_{v \in \mathcal{H}_d} \mathcal{L}^-_{\{x\in Q_v\notin Z\}}(g') - \mathcal{L}^-_{\{x\in Q_v\notin Z\}}(g) +\mathcal{L}^-_{\{x\in E_v\}}(g') - \mathcal{L}^{-}_{\{x\in E_v\}}(g).   $$

Now, for each event $\{x \in Q_v\notin Z
\}$, we consider two cases depending on the number of negative samples in $Q_v$. (1) If there is at least one negative sample $x_i^- \in Q_v$, then
$g'(x)= g'(x_i^-) = g(x) = g(x_i^-)$, so both the log-sums in $\mathcal{L}^-_{\{x\in Q_v\notin Z\}}(g')$ and $\mathcal{L}^-_{\{x\in Q_v\notin Z\}}(g)$ are dominated by $e^{\beta d}$ terms and the losses do not significantly differ (using that log-sum is approximately a max operation). (2) If no negative samples lie in $Q_v$, then the dominant terms in the log-sum for $\mathcal{L}^-_{\{x\in Q_v\notin Z\}}(g')$ may be a factor of $e^{2\beta}$ larger than the dominant terms for $\mathcal{L}^-_{\{x\in Q_v\notin Z\}}(g)$, requiring a sharp analysis to control the probability   these events occur.
Letting $n_{1,v}$ denote the number of negative samples in $Q_v$, we define these two  cases above  as $B_{v,1}\coloneqq\{x \in Q_v \notin Z, n_{1,v}>0\}$ and $B_{v,2
}\coloneqq \{x \in Q_v \notin Z, n_{1,v}=0\}$, respectively. Note that they form a partition of $\{x \in Q_v\notin Z\}$, so we have $\mathcal{L}^-_{\{x\in Q_v\notin Z\}}(g') - \mathcal{L}^-_{\{x\in Q_v\notin Z\}}(g) = \sum_{j=1}^2 \mathcal{L}^-_{B_{v,j}}(g') - \mathcal{L}^-_{B_{v,j}}(g)$. 
We detail each case below, where $n_2$ is the number of negative samples in $E$. 



% Let 
% We define the intersection of the negative loss with the event $B\coloneqq B(x,x^+, \{x^-_i\}_{\ell})$ as:
% $$\mathcal{L}_{B}^-(g)\coloneqq \mathbb{E}_{x,x^+, \{x^-_i\}_{\ell}} \bigg[ \chi \{B(x,x^+, \{x^-_i\}_{\ell})\}  \log\bigg({ e^{\beta g(x)^\top g(x^+)}+\sum_{i=1}^\ell e^{\beta g(x)^\top g(x^-_{i})}  } \bigg)\bigg] $$ where $\chi \{\cdot\} $ is the indicator function. Using this definition, we can leverage the partition of the space of images defined above to write the difference in negative parts of the loss as the sum over the differences in negative parts of the loss intersected with the events $\{x \in Q_v\}$ and $\{x \in E_v\}$ for all vertices $v$. 

% Formally, we have


% Next, we note that we only need to consider intersections with $\{x\in $






% Thus we iterate over $v \in \mathcal{H}_d$, and for each $v$, consider four cases, two corresponding to $x \in Q_v \notin Z$ and two to $x \in E_v$. These sets of two cases are roughly symmetric, so we only consider $x \in Q_v\notin Z$ here. Central to these two cases are the number of negative samples in $Q_v$ and $E$, defined as $n_{1,v}$ and $n_2$, respectively. 


% Indeed, for 
% $x \in Q_v\notin Z$, we can characterize the behavior of $g'(x)^\top g'(x_{i}^-)$ and $g(x)^\top g(x_{i}^-)$  depending on whether $x_i^-$ lies in $Q_v, E$, or $D\setminus (Q_v\cup E)$: $(i)$ $x_i^-\in Q_v \implies g'(x)^\top g'(x_{i}^-) = g(x)^\top g(x_{i}^-) = d$ by definition of $Q_v$, $(ii)$ $x_i^-\in E \implies g'(x)^\top g'(x_{i}^-) = g(x)^\top g(x_{i}^-) + 2$ by definition of $E$ and $Z$, and $(iii)$  $x_i^- \in D\setminus (Q_v\cup E) \implies g'(x)^\top g'(x_{i}^-) = g(x)^\top g(x_{i}^-)$. Using these observations, we analyze the following two cases.

 % We have: 
% we split the negative losses on the events

% $\mathcal{L}_{\text{neg}, E}\coloneqq \mathbb{E}_{x,x^+, \{x^-_i\}_{\ell}} \bigg[ \chi \{x \in Q_v\}  \log\bigg({ e^{\beta g(x)^\top g(x^+)}+n_{1,v}e^{\beta d}+ \sum_{x_i^{-} \in B}e^{\beta g(x)^\top g(x^-_{i})} 
%  +\sum_{x_i^{-}\not\in {A}_v\cup B} e^{\beta g(x)^\top g(x^-_{i})}  } \bigg)\bigg] $

% In comparing $\mathcal{L}(g)$ to $\mathcal{L}(g_c)$, the positive term in Equation (\ref{eq:InfoNCE}) increases by exactly $$2\beta \left(\Pr\left[x\in A, x^+\in B\right] + \Pr\left[x\in B, x^+\in A\right]\right),$$ while the negative term can be shown to decrease by no more than this quantity by considering three cases for each $v\in \mathcal{H}_d$: 

% PLAN: 

% can possibly delete Theorem 9 (it is almost trivial)
% maybe we don't need technical figure for clusters
% todo: clean up circ vs non-circ notations
% check other proofs
% For proof sketch:
% define n1v, n2, etc? or just focus high-level on the bad cases?
% need to explain why regularity assumption is important.
% need to explain when negative loss can get worse, when it can improve.
% need to explain choice of large ell and beta.
% can delete remark on representations on thehpercube

% $$\mathcal{L}_{E}\coloneqq \mathbb{E}_{x,x^+, \{x^-_i\}_{\ell}} \bigg[ \chi \{E\}  \log\bigg({ e^{\beta g(x)^\top g(x^+)}+n_{1,v}e^{\beta d}+ \sum_{x_i^{-} \in B}e^{\beta g(x)^\top g(x^-_{i})} 
 % +\sum_{x_i^{-}\not\in {A}_v\cup B} e^{\beta g(x)^\top g(x^-_{i})}  } \bigg)\bigg] $$

% {\color{red}
% \item \textbf{Case 1:} $E_1 := \{x \in Q_v \notin Z, n_2=0\}$. In this case, $g'(x)^\top g'(x_{i}^-) = g(x)^\top g(x_{i}^-)$ for all $i \in [\ell]$, so the negative loss increases for $g'$  iff  $x^+\in B$. We obtain:
% $\mathcal{L}_{E_1}^-(g')- \mathcal{L}_{E_1}^-(g) \leq 2 \beta \mathbb{P}(x \in Q_v \notin Z, x^+\in B, n_2=0, n_{1,v}=0 ) + \log(2)\mathbb{P}(x \in Q_v \notin Z, x^+\in B, n_2=0, n_{1,v}>0 )$. 
% % $\mathcal{L}_{E_1}^-(g')- \mathcal{L}_{E_1}^-(g) \leq \mathbb{E}[\chi\{E_1\} \log\left(\frac{ e^{\beta g(x)^\top g(x^+)} + n_{1,v}e^{\beta d} }{ e^{\beta g(x)^\top g(x^+)} + n_{1,v}e^{\beta d}  } \right)]$ 



% % $\{x\in A, x^+\in A\}$. These contribute $l\Vert B\Vert_\circ$ - that is, roughly a contribution of $1$ in the event that even a single negative sample is drawn from the region $B$.

% \item \textbf{Case 2:} $E_2 := \{x \in Q_v\notin Z, n_2>0, n_{1,v}=0\}$. %$x \in Q_v, n_2 >0, n_{1,v}=0$. In this
% Here we may have  $g'(x)^\top g'(x_{i}^-) = g(x)^\top g(x_{i}^-) +2$ for all $i \in [\ell]$ if $Q_v\cup B = D$, i.e. at worst all negative pairs can have inner product larger on $g'$ by 2 compared to $g$. Thus the loss may increase by (at most) $2\beta \mathbb{P}(x \in Q_v\notin Z,n_{1,v}=0)$. 


% \item \textbf{Case 3:} $E_3 := \{x \in Q_v\notin Z, n_2>0, n_{1,v}>0\}$. In this case, the $n_2$ negative pairs with $x_{i}^-\in B$ have increased similarity, but this increase is buffered by the presence of negative samples in $Q_v$ that incur $e^{\beta d}$ terms for both $g$ and $g'$. At worst, we have
% \begin{align}
%     \!\mathcal{L}_{E_3}^-(g')\!- \!\mathcal{L}_{E_3}^-(g) \!\leq \mathbb{E}\big[\chi\{E_3\} \log\big(\tfrac{ n_{1,v}e^{\beta d} + (n_2+1)e^{\beta d} }{n_{1,v}e^{\beta d} + (n_2+1)e^{\beta (d-2)}} \big) \big] \leq \mathbb{E}\big[\chi\{E_3\} \log\big(\tfrac{ n_{1,v} + n_2 + 1 }{n_{1,v}} \big) \big] \nonumber
% \end{align}
% % The rightmost expression does not depend on $\beta$, so naively we could bound $n_{1,v}+n_2\leq \ell$ to obtain  $\mathcal{L}_{E_3}^-(g')\!- \!\mathcal{L}_{E_3}^-(g) \leq \mathbb{P}(x \in Q_v)\log(\ell+1) \ll \beta$ for large enough $\beta$. However, this bound would not depend on $\|R\|$, so it may exceed $\Lambda^+$. To address this, 
% We bound $\log\big(\tfrac{ n_{1,v} + n_2 + 1 }{n_{1,v}} \big) \leq \frac{2 (n_2+1)}{n_{1,v}}$. Intuitively, this should scale with the ratio $\frac{\|B\|_\circ}{\|Q_v\|_\circ}$ by the definitions of $n_2$ and $n_{1,v}$. We show that this is indeed the case by completing a trinomial expansion, resulting in $\mathbb{E}\big[\chi\{E_3\}\tfrac{n_2+1}{n_{1,v}}\big]= O(\|B\|_\circ)=  O(\|R\|)$ by Assumption \ref{assump-b}.
% }

% can choose beta >= \min ( 2^d log(1/epsilon), d/epsilon)
 \textbf{Case 1:} $B_{1,v} := \{x \in Q_v \notin Z, n_{1,v}>0\}$. In this case %$ g'(x)^\top g'(x_{i}^-) = g(x)^\top g(x_{i}^-) = d$ for at least one $i \in [\ell]$, meaning that
the dominant terms in the log sums for $\mathcal{L}^-_{B_{1,v}}(g')$ and $\mathcal{L}^-_{B_{1,v}}(g)$ are both $e^{\beta d}$, although the losses may  differ in the number of such terms, which can be, in the worst case, $n_{1,v}+n_2+1$ for $g'$ and $n_{1,v}$ for $g$. This is because  $g$ and $g'$ can disagree on at most $n_2$ negative samples, and they can also disagree on the positive sample. Thus, $\!\mathcal{L}_{B_{1,v}}^-(g')\!- \!\mathcal{L}_{B_{1,v}}^-(g) \! \leq \mathbb{E}\big[\chi(B_{1,v}) \log\big(\tfrac{ n_{1,v} + n_2 + 1 }{n_{1,v}} \big) \big]  \leq \mathbb{E}[\chi(B_{1,v}) \frac{2(n_2+1)}{n_{1,v}+1}]$, where the last inequality follows using $\log(1+x) \leq x$.                                                                                    
% If $n_2=0$ then the loss of $g'$ can only increase if $x^+\in B$, and a simple calculation shows that $\mathcal{L}_{E_1\cap \{n_2=0\}}^-(g') - \mathcal{L}_{E_1\cap \{n_2=0\}}^-(g)\leq \log(2) \mathbb{P}(x\in Q_v, x^+ \in B) \mathbb{P}(n_{1,v}=0, n_2=0)$. For general $n_2$ we can show that 
% \begin{align}
%     \mathcal{L}_{E_1}^-(g') - \mathcal{L}_{E_1}^-(g)\leq \mathbb{E}\big[ \chi\{E_1\} \log( ) \big] 
% \end{align}
% \begin{align}
%     \!\mathcal{L}_{B_{v,1}}^-(g')\!- \!\mathcal{L}_{B_{v,1}}^-(g) \!\leq \mathbb{E}\big[\chi\{B_{v,1}\} \log\big(\tfrac{ n_{1,v}e^{\beta d} + (n_2+1)e^{\beta d} }{n_{1,v}e^{\beta d} } \big) \big] \leq \mathbb{E}\big[\chi\{B_{v,1}\} \log\big(\tfrac{ n_{1,v} + n_2 + 1 }{n_{1,v}} \big) \big], \nonumber
% \end{align}
% where $ \log\big(\tfrac{ n_{1,v} + n_2 + 1 }{n_{1,v}} \big)\leq \frac{2(n_2+1)}{n_{1,v}+1}$ using $\log(1+x) \leq x$.  
We bound $\mathbb{E}[\chi(B_{1,v}) \frac{2(n_2+1)}{n_{1,v}+1}]$ by writing the trinomial expansion of the expectation (note that the joint distribution of ($n_{1,v},n_2$) is trinomial with parameters ($\|Q_v\|_\circ, \|E\|_\circ$)), 
% and factoring the $n_2$ and $n_{1,v}+1$ terms to obtain a new trinomial 
and further simplifying to result in an upper bound of $\|E\|_\circ$. Importantly, this bound is  $O(\|R\|)$ by Assumption \ref{assump-b} and independent of $\beta$, so we control it by making $\beta$ large enough. 
% Note that this analysis avoids requiring scaling $\beta$
% inversely with $\|R\|$.


% Thus, a naive bound gives $$\mathcal{L}_{E_1}^-(g')- \mathcal{L}_{E_1}^-(g) \leq \mathbb{E}\big[\chi\{E_1\} \log\big(\tfrac{ (\ell+1)e^{\beta d}  }{ n_{1,v}e^{\beta d}} \big) \big]\leq \mathbb{P}(x\in Q_v\notin Z)\log(\ell+1),$$ 
% where the RHS is $O(\beta \|R\|)$ for sufficiently large $\beta$. We give a more fine-grained analysis to avoid scaling  $\beta$ with $1/\|R\|$. 

\textbf{Case 2:} $B_{2,v} := \{x \in Q_v \notin Z, n_{1,v}=0\}$. 
Since here there is no shared dominant $e^{\beta d}$ term in the log-sums for $\mathcal{L}^-_{B_{2,v}}(g')$ and $\mathcal{L}^-_{B_{2,v}}(g)$, the dominant terms for $g'$ may involve strictly larger similarities than those for $g$, corresponding to $x_i^- \in E$ and $x^+ \in E$ (the only samples on which $g'$ and $g$ can disagree).
% Specifically, the loss for $g$ may be up to a factor $2\beta$ larger than the loss for $g$ for some batches  $(x,x^+,\{x_i^-\}_\ell)$, which means that $\mathcal{L}_{B_{v,2}}^-(g')- \mathcal{L}_{B_{v,2}}^-(g)$ is up to $2\beta$ times the probability that these batches are drawn. 
These events are bounded depending on whether $n_2=0$. If $n_2=0$, the loss of $g'$ exceeds that of $g$  iff $g'(x)^\top g'(x^+) = g(x)^\top g(x^+) + 2$, which occurs iff $x^+ \in E$. 
% Thus  $\mathcal{L}_{\{x \in Q_v \notin Z, n_1=0,n_2=0\}}^-(g') - \mathcal{L}_{\{x \in Q_v \notin Z, n_1=0,n_2=0\}}^-(g)\leq 2\beta \mathbb{P}(x \in Q_v, x^+ \in B) \mathbb{P}(n_{1,v}=0,n_2=0)$. 
% For $n_2 >0$, a similar argument shows that $\mathcal{L}_{\{x \in Q_v \notin Z, n_1=0,n_2>0\}}^-(g') - \mathcal{L}_{\{x \in Q_v \notin Z, n_1=0,n_2>0\}}^-(g)\leq 2\beta \mathbb{P}(x \in Q_v) \mathbb{P}(n_{1,v}=0,n_2>0)$.
If $n_2 >0$, the loss can increase by $2\beta$ regardless of the value of $x^+$. 
Combining these sub-cases yields
\begin{align}\mathcal{L}_{B_{2,v}}^-(g') - \mathcal{L}_{B_{2,v}}^-(g)&\leq 2\beta \mathbb{P}(x \in Q_v\notin Z, x^+ \in E) \mathbb{P}(n_{1,v}=0,n_2=0) \nonumber \\
&\quad + 2\beta \mathbb{P}(x \in Q_v\notin Z) \mathbb{P}(n_{1,v}=0,n_2>0). \nonumber
\end{align}
For each term above, we need to show that the coefficient of $2\beta$ is $o(\|R\|)$ even after it is summed over $v$. Note that both terms scale with the probability that $x \in Q_v \notin Z$ {\em and} no negative samples are in $Q_v$. To control this probability we leverage that the distribution induced by $g$ is close to uniform in the sense that every ``active'' vertex $v$ has mass $\mathbb{P}[g(x)=v]=\tilde{\Omega}(\frac{1}{d2^d})$. We use this fact to bound $\mathbb{P}[x \in Q_v]$. Note that the set of images that $g$ maps to $v$ is $Q_v \cup E_v$, yet for all $Q_z \notin Z$, $E_v=\emptyset$ since, at a high level, $f_1$ must separate these $Q_v$ from $E$. So, $\mathbb{P}[g(x)=v] = \mathbb{P}[x \in Q_v]$ for all $Q_v\notin Z$. Therefore, we can show that  with large $\ell$  it is highly unlikely that $x\in Q_v \notin Z$ and none of the negative samples are in $Q_v$. To complete the bounds, we leverage the facts that  $\mathbb{P}[x \in Q_v\notin Z, x^+ \in E]$ scales with $\|R\|$ for the first term, and $\mathbb{P}[n_2>0]$ scales with $\|E\|_\circ$ for the second term, where $\|E\|_\circ = O(\|R\|)$ by Assumption \ref{assump-b}.
% To bound the second term, we again leverage the observation that 
% the second term does not grow with $\beta$ and can be dominated by $\beta$ large enough. The first term


% $g'(x)^\top g'(x_{i}^-) = g(x)^\top g(x_{i}^-) +2$ for all $i \in [\ell]$ if $Q_v\cup B = D$, i.e. at worst all negative pairs can have inner product larger on $g'$ by 2 compared to $g$. Thus the loss may increase by (at most) $2\beta$ times the probability that . 

% \begin{align}
%     \!\mathcal{L}_{E_1}^-(g')\!- \!\mathcal{L}_{E_1}^-(g) \!\leq \mathbb{E}\big[\chi\{E_3\} \log\big(\tfrac{ n_{1,v}e^{\beta d} + (n_2+1)e^{\beta d} }{n_{1,v}e^{\beta d} + (n_2+1)e^{\beta (d-2)}} \big) \big] \leq \mathbb{E}\big[\chi\{E_3\} \log\big(\tfrac{ n_{1,v} + n_2 + 1 }{n_{1,v}} \big) \big] \nonumber
% \end{align}

% and choose $\beta > \log(\ell+1)$ large enough to try to ensure 

% $\mathcal{L}_{E_3}^-(g')\!- \!\mathcal{L}_{E_3}^-(g) $ 

% is less than $\Lambda^+$
% $\{x\in A, x^+\in B\} \bigcup \{x\in B, x^+\in A\}$. These contribute $2\beta +\log \ell$ - that is, roughly a contribution of $2\beta$ in the event that no negative sample is drawn from the same set as $x$, and no more than $\log l$ otherwise.
% \item $\{x\in B, x^+\in B\}$. These contribute $l\Vert A\Vert_\circ$ - that is, roughly a contribution of $1$ in the event that even a single negative sample is drawn from the region $A$.
% \item $\{x\in C\}$. These only increase the negative loss.
 
% To summarize, in the regime $\log \ell < 0.1\beta$, this means that the positive term increases by more than the negative term decreases when switching from $g$ to $g'$. A detailed proof is given in Appendix \ref{appendix:oned}.

After performing a similar analysis for $\{ x \in E_v\}$ and summing the resulting bounds over $\{v \in \mathcal{H}_d\}$, as in \eqref{eq:sumv},  we obtain $\mathcal{L}^-(g') - \mathcal{L}^-(g)< 2 \beta \|R\| = \mathcal{L}^+(g) - \mathcal{L}^+(g')$.
\begin{comment}
{\color{gray}
Note that the two events above form a partition of $\{x \in Q_v\notin Z\}$, i.e. $\mathcal{L}^-_{\{x\in Q_v\notin Z\}}(g') - \mathcal{L}^-_{\{x\in Q_v\notin Z\}}(g) = \sum_{j=1}^2 \mathcal{L}^-_{B_j}(g') - \mathcal{L}^-_{B_j}(g)$. After summing over $\{v \in \mathcal{H}_d: Q_v\notin Z\}$ and performing a similar analysis for $\{ x \in E_v\}$, we obtain
\begin{align}
    \mathcal{L}^-(g') - \mathcal{L}^-(g) &\leq  2\beta \sum_{v: Q_v \notin Z} \big(\mathbb{P}(x \in Q_v \cap x^+ \in E) (1 - \|Q_v\|_\circ)^\ell   +   \ell \|B\|_\circ \|Q_v \|_\circ (1 - \|Q_v \|_\circ)^{\ell-1} \big)\nonumber\\
&\quad +  2\beta \sum_{v\in \mathcal{H}_d} \|E_v\|_\circ (1 - \|E_v\|_\circ)^\ell  + o(\beta \|R\|)  \nonumber
    % \|Q_v\|_\circ(1 - \|Q_v\|_\circ - \|B\|_\circ)^\ell + 
\end{align}
To bound the RHS, we leverage $g$ being close to uniform to upper bound $\sum_{v \in \mathcal{H}_d: Q_v \notin Z} \|Q_v \|_\circ (1 - \|Q_v \|_\circ)^{\ell-1}$, noting that $\mathcal{D}_g(v) = \|Q_v\|_\circ$ iff $Q_v \notin Z$. Finally, we show that $\sum_{v \in \mathcal{H}_d} \mathbb{P}(x \in Q_v \cap x^+ \in B) (1 - \|Q_v\|_\circ)^\ell \lesssim \frac{\|R\|}{e}$,  and  $\sum_{v \in \mathcal{H}_d} \|E_v\|_\circ (1 - \|E_v\|_\circ)^\ell\lesssim \frac{\|E\|_\circ}{e} \leq \frac{\|R\|}{\delta e}$ (by Assumption \ref{assump-b}), meaning that $\mathcal{L}^-(g') - \mathcal{L}^-(g) < \mathcal{L}^-(g) - \mathcal{L}^+(g') $ for $\delta \geq 0.6$, completing the proof. }
% {\color{red} need to use Weighted InfoNCE loss?}
\end{comment}

\end{proof}

Theorem \ref{thm:agnostic} shows that for large $\ell$ and $\beta$, all minimizers of the InfoNCE loss that are near-uniform must be cluster-preserving regardless of the sizes of each cluster or the number of clusters. 
% Combined with Lemma \ref{lemma:entropy}, which shows that the InfoNCE loss almost behaves like the Shannon entropy and therefore encourages uniform representations, Theorem \ref{thm:agnostic} suggests that  in the agnostic case. 
However, it does not rule out that there could be a highly non-uniform and non-cluster-preserving optimal representation. In Appendix \ref{app:weighted}, we show that if we re-weight the alignment and uniformity losses in the InfoNCE loss, we can ensure that {\em all} minimizers of the InfoNCE loss are cluster-preserving.

% {\color{red} define near-uniform formally before theorem statement?}

% Discussion of why this result is significant? 



% Weighted InfoNCE loss for non-uniform distributions. 

% {\color{red}Finally, we have the following Lemma that states that, among clean representations, the InfoNCE loss maximizes the entropy of the pre-trained representations when $l=\{1, 2\}$. Note that the result is similar to that of Lemma \ref{thm:uniform}, however we can completely characterize the ordering on distributions in this case and the the proof is specific to $d=1$ (Lemma \ref{thm:uniform} only holds for $d>4$). 

% \begin{lemma}
%     Equation (\ref{eq:Ltilde}) is minimized by the clean representation $g$ that induces a distribution $\mathcal{D}_g$ with maximal entropy.
% \end{lemma}
% The proof follows by writing out the loss explicitly and optimizing over the one parameter family of distributions of Rademacher random variables, and is provided in Appendix~\ref{appendix:maxentropy}.}






==> Spiky Augmentations/Theory/Bias.tex <==
%% \subsection{Clus}

The goal of contrastive learning is to learn a representation from unlabeled samples that is useful for downstream tasks. Recall that the representations we consider map images to vertices on the Rademacher hypercube $\mathcal{H}_d$. A ``good'' representation should map images from the same cluster to the same vertex, and images from distinct clusters to distinct vertices.

% We consider a class of representations consisting of concatenated binary classifiers, with the classification boundaries of two example classifiers shown above ($f_1$ and $f_2$). The classifiers have limited complexity, which respects an clustering of images and their augmentations. Specifically, clusters are sets of images such that are not split by any ``clean'' classifier that does not pass through any augmentation set,  e.g. $f_1$ in the figure. Thus, if a classifier intersects a cluster, then it must also intersect at least one augmentation set, e.g. as the non-clean classifier $f_2$ intersects the blue and green augmentation sets in the Dogs cluster. Our motivating assumption is that the underlying clusters are related to downstream tasks.

Intuitively, this seems possible if images having the same content (i.e., from the same cluster) along with their set of augmentations are ``close and intertwined'' (see Figure~\ref{fig:spiky}), such that any function $f \in \F$ cannot split the cluster without also splitting an image from its augmentation.
Note that we do {\em not} need connected clusters with overlapping augmentations (meaning two images have the same augmentation, which is an unrealistic assumption); merely that the cluster has a complex geometry relative to the function class. 
%We formalize this through `cleanness' of representations.

%% The representation $g \in G$ should 

\subsection{Complexity of $\mathcal{F}$ Relative to Augmentations}
\label{sec:cluster-bias}
%% Our setting is one consisting of natural images and their augmentations (crops, rotations, etc.).  

%% The fundamental mystery of contrastive learning is the ability of pretrained representations to learn useful concepts from data without   labels. Consider the following simplified example. Suppose there are only four (unlabeled) natural images: two images of  cats, and two images of dogs. We can augment these images as desired using crops, rotations, etc. to construct new images; however we will never truly get the {\em same} new image as an augmentation of two different original images. In other words, the augmentation sets corresponding to distinct natural images are generally disjoint, a problem first highlighted by \citet{saunshi2022understanding} and further addressed by \citet{haochen2022beyond}. Due to the disjointness of augmentation sets, there is no immediate formal sense in which the first natural image of the cat is any more similar to the other image of a cat than either of the dog images, so it is not clear how unsupervised pretraining can learn any meaningful relationships between the images. If our downstream task consisted of distinguishing cats and dogs, why would pretraining help? 

%% We approach the resolution of this question by first considering a thought experiment. Imagine a fully supervised version of the downstream task that is trained with access to natural and augmented, \textit{labeled} images. For this supervised learning task to be solvable at all, it must be true that the function class $\F$ contains an inductive bias that allows the learner to learn some functions of the data and not others. The same is true for the unsupervised setting -- if we hope to learn meaningful representations, the representation class must only allow for learning a particular set of representations.

% Recall that $\F$ is a class of binary-valued functions with bounded expressivity. 



%\begin{comment}
\begin{figure}
  \begin{minipage}[c]{0.45\textwidth}
    % \includegraphics[height=1.9in,width=3in]{spikyaugs2.pdf}
    \vspace{-4mm}
    \includegraphics[height=2.2in,width=2.5in]{spikyaugs2.pdf}
  \end{minipage}\hfill %\hspace{-0.5in}
  \begin{minipage}[c]{0.55\textwidth}
\caption{We illustrate a setting with four clusters, and two augmentation sets within each cluster indicated by linked rectangles in distinct colors. The clean function $f_1$ does not split any augmentation or cluster (meaning, it maps all images from the same augmentation set alike, and likewise for clusters). $f_2$ splits the cluster of dogs, and in accordance with Assumption~\ref{assump:spikyaug}, also splits augmentation sets within that cluster (and is therefore non-clean).
% augmentation of one of the natural dog images, and also split the cluster of dogs (two natural dog images are split). 
Finally, $f_3$ violates Assumption~\ref{assump:spikyaug}, because it does not split any augmentation of pandas, yet it splits the pandas cluster.
Images are from the Animals V2 dataset: \cite{deepnets_2022}.\label{fig:spiky}}
\end{minipage}
\end{figure}
%\end{comment}

We formalize the notion of bounded expressivity of $\F$  relative to the geometry of clusters.
% through an assumption on the spikyness of ``clusters''.
% in the form of clusters.
% We now show that the classifier class $\mathcal{F}$ induces a clustering of images from possibly different augmentation sets, as discussed in the Introduction {\color{blue} [KS: This sentence does not read right. We want to say about an inductive bias assumption not a result we establish]}. 
We use this assumption to show in Section \ref{sec:realizable} that solutions to the InfoNCE loss optimized over $\mathcal{G}$ satisfy useful uniformity and alignment properties that lead to downstream performance guarantees on tasks that adhere to the clusters. 
%
% \textbf{Inductive bias in the form of clusters.} 
% We show that the representation class $\G$ inherits a natural inductive bias of the classifier class $\mathcal{F}$ in our setting with augmentations rather than labels. 
% The inductive bias of $\mathcal{F}$ consists of the data clusters that can result from classifiers in $\mathcal{F}$ that are ``clean'' with respect to augmentation sets.
% as illustrated in Figure \ref{fig:clean}. 
Formally, the function class $\F$ and the augmentations $\Lambda$ define a set of \textit{clean} functions $\F_c \subseteq \mathcal{F}$ that separate the data in a way that respects the augmentations. % 

\begin{definition}[Clean Function]
% \begin{align} 
%% f\in \F_c\iff f(\I(\lc, \ls)) = f(\I(\lc, \ls'))~\forall  %\ls, \ls'\in S. 
$f\in \F_c \ \ {\rm{is \ clean}} \ \iff f(x) = f(\mathcal{A}(x)))~\forall x \in  D_\circ,  \mathcal{A} \in \Lambda$. % \ls, \ls'\in S. 
\label{eq:defclean}
% \end{align}
\end{definition}
In other words, the binary function $f$ is clean if it does not separate any image and its augmentations from each other. 
% {\color{red} Note that $\mathcal{F}$ induces a bias of contrastive learning solutions  towards the set of clean classifiers $\mathcal{F}_c$, since contrastive learning aims to preserve alignment of augmentation sets.} 
Our main assumption is that if a classifier in $\mathcal{F}$ splits a cluster, then it is not clean.
% the clean classifiers in $\mathcal{F}_c$ are consistent with the underlying clusters in the data due to intertwined augmentations.
\begin{assumption}[Intertwined Augmentations] \label{assump:spikyaug}
% $f \in \mathcal{F}_c \iff f(x)= f(x') \; \forall \; x,x'\in \Gamma_{\mathbf{c}}\; \forall \; \mathbf{c} \in C$.
For all $f \in \mathcal{F}$, if $f(x)\neq f(x')$ for some $x,x'\in \Gamma_{\mathbf{c}}$, then $f(x'')\neq f(\mathcal{A}(x''))$ for some $x'' \in \Gamma_{\mathbf{c}} \cap D_{\circ}$, where $\mathcal{A}(x'') \in {A}(x'')$.
\end{assumption}
Note that if a classifier does not split any cluster, then it must be clean, since augmentation sets are contained within clusters. Thus, 
Assumption \ref{assump:spikyaug} implies that
% states that if 
% $f\notin \mathcal{F}_c$ splits natural images in a cluster then it must also split an augmentation set for some natural image in  that cluster. 
% In other words,  
$f \in \mathcal{F}_c$ if and only if $f$ labels all images with the same content (belonging to the same cluster) alike, in other words it is \textit{cluster-preserving}. 
This assumption holds if the augmentation sets within clusters are close and intertwined (they cannot be easily split from the rest of the cluster), relative to the complexity of $\mathcal{F}$. Importantly, the augmentation sets need not overlap, meaning a single image need not be an augmentation to multiple natural images, consistent with practice \citep{saunshi2022understanding}.
%
As prior works have pointed out \citep{saunshi2022understanding,haochen2022theoretical}, Assumption \ref{assump:spikyaug} or variants on the bounded complexity of the function class are necessary for the success of CL in the realistic setting in which the augmentation sets do not overlap.
%
% Consider the example in Figure \ref{fig:spiky}. There are images of cats, dogs, pandas and cows, each with augmentation sets indicated by colors. Here the clusters relevant to downstream tasks are the four classes of images, and are indicated by dotted black circles.  Note that the augmentation sets within each cluster do not overlap, consistent with practice \citep{saunshi2022understanding}. This means that a complicated classifier $\bar{f}$ can split two augmentation sets within a cluster  from each other without splitting any image from any of its augmentations. If CL were allowed to incorporate such classifiers into its representation, it might do so, since they are perfectly aligned (i.e maximize similarity between represented images and their augmentations) while also help to minimize similarity between negative samples, as they treat negative samples within the same cluster differently. However, employing such classifiers does not lead to useful representations, since images from the same cluster and thereby sharing the same label on downstream tasks are represented differently (mapped to different vertices on the hypercube). Thus, we need to assume the function class has limited complexity relative to the augmentations such that classifiers such as $\bar{f}$ are not admitted.  Indeed, such an assumption is natural as augmentation sets are highly non-smooth in Euclidean space, as they typically consist of rotations, crops and color transformations that map the natural image in a non-local manner. We formally prove that Assumption \ref{assump:spikyaug} is necessary to achieve meaningful downstream guarantees in Theorem \ref{thm:negative}.

However, while some condition like Assumption \ref{assump:spikyaug} is necessary, it is not clear if this suffices to show that CL learns useful representations. Consider the example in Figure \ref{fig:spiky}. 
% There are images of cats, dogs, pandas and cows, and the augmentation sets are sufficiently spiky relative to the function class  $\mathcal{F}$ such that any classifier in $\mathcal{F}$, e.g. $f_2$, that splits a cluster must also split an augmentation set within that cluster. 
% Note that $\bar{f}$ does not belong to $\mathcal{F}$ according to Assumption \ref{assump:spikyaug}.  Still, 
It may be the case, for instance, that CL on $\mathcal{F}$ does not learn the cluster-preserving classifiers, as in addition to trying to maximize the similarity between  images and their augmentations, CL also tries to minimize the similarity between negative pairs of images.  Thus, it may choose a non-cluster-preserving classifier such as $f_2$ in an effort to minimize similarity of negative pairs. This would lead to poor downstream generalization on tasks involving classifying dogs, since $f_2$ separates images of dogs. It thus becomes critical to quantify the extent to which non-cluster-preserving classifiers must intersect augmentation sets such that CL will not learn them, as we do in Section \ref{section:agnostic}. Before this, we must show that even if CL learns a representation consisting of cluster-preserving classifiers, this representation generalizes well, which may not happen if it maps two or more clusters to the same vertex.
For instance, if CL simply learned $d$ copies of the cluster-preserving classifier $f_1$ in Figure \ref{fig:spiky}, this representation would not be able to distinguish cows from pandas from dogs on downstream tasks. We thus desire representations to be {\em  both} cluster-preserving and uniform  such that their mapping is a bijection from clusters to vertices. Next, we show that when a cluster-preserving and uniform representation is realizable, CL with the InfoNCE loss learns it, even with finite negative samples per batch.



% This is because CL trades off between uniformity and alignment, so it may choose non-clean classifiers to compose optimal representations in pursuit of uniformity.





%%%% {\color{blue} Aryan, Karthikeyan: please do not edit above. This is still work in progress. Thanks. Sanjay}

% For example, Figure \ref{fig:cleanb} shows all classifiers in $\mathcal{F}$, while Figure \ref{fig:cleanc} shows only the classifiers in $\mathcal{F}_c \subset \mathcal{F}$. Notice that that classifiers in $\mathcal{F}_c$ induce a clustering of images is illustrated in Figure \ref{fig:cleanc}.
% This bias is formalized via our definition of clean classifiers and is illustrated in 
\begin{comment}
\begin{figure}[t]
\centering
\resizebox{5cm}{!}{\input{}}
\caption{
}\label{fig:clean}
\end{figure}
\end{comment}
% \textbf{Clusters and inductive bias of function class.}
% Together,  
% Using the above definition of $\mathcal{F}_c$ in \eqref{eq:defclean}, we define an equivalence relation $\equiv$ between content variables that captures the notion that some pairs of content variables are always classified alike for all clean functions.
% \begin{align}\label{eq:equivalencerelation}
% \lc\equiv \lc'\!\iff \!\forall f\in \F_c, \forall \ls, \ls'\in S, f(\I(\lc, \ls)) \!=\! f(\I(\lc', \ls')) \nonumber
% \end{align}
% We denote the equivalence set for an image $\I(\lc, \ls)$ as $\Gamma_{\lc} = \{\I(\lc', \ls')| \lc' \equiv \lc\}$ and 
% refer to this set as the \textit{cluster} of image $\I(\lc, \ls)$. Likewise, $\Gamma_{\lc,\circ} = \{\I(\lc', \ls')| \lc' \equiv \lc,\ls'\in {S}_\circ\}$ is the set of all natural images in the cluster $\Gamma_{\lc}$. We overload the use of the equivalence relation also for images, so $x\equiv x'$ if and only if $\lc\equiv \lc'$ where $x = \I(\lc, \ls)$ and $x' = \I(\lc', \ls')$. In other words, two images belong to the same cluster if and only if there is no clean function that can separate them or any of their augmented images. {We denote $m := m(\mathcal{F}_c, {D})$ as the number of distinct clusters in the dataset}.

% {\color{blue} The inductive bias in the function class ${\cal F}$ is specified through the equivalence class of images under the equivalence relation $\equiv$ that are not separable by any clean function. In other words, if two images with different content components within an equivalence class is separated by any function $f \in {\cal F}$, then the function $f$ is not \textit{clean}, i.e. it must separate some image and its augmentation as well. As long as there is an equivalence class containing distinct content components, then the inductive bias imposed in non trivial.}
%
%{\color{blue} [KS: Downstream stuff + assumption 1 could be moved to Section 4.3. Otherwise it breaks the flow ]}
%\textbf{Downstream tasks.} Our main assumption is that downstream tasks label all images from the same cluster alike, hence the clusters are meaningful for downstream performance.
%\begin{assumption}[Meaningful clusters] \label{assump:downstream}
%The set of downstream tasks $\mathcal{T}$ is a subset of $\mathcal{F}_c$.
%\end{assumption}
%
% Thus, the bias induced by the function class leads to clusters that are \textit{meaningful} in the sense that they align with downstream tasks. 
%
% similar to the one made by \citet{haochen2022theoretical}
% Note that  if generalization error is characterized by error on augmentations, then only clean tasks can have generalization guarantees using our function class $\F$  since for every function $f\in \F\setminus \F_c$ there is some image $x$ and augmentation $A$ such that $f(x) \ne f(A(x))$.

% Finally, a clean representation $g \in \mathcal{G}_c$ is one that is a concatenation of $d$ clean functions from $\mathcal{F}_c$.

%  %We show that pretraining using augmentations allows us to learn a representation such that each coordinate respects the augmentations.
% % {\color{red} (that is, which is like the green classifier above)}. 
% %We refer to such classifiers, and such representations, as \textit{clean}. 
% \begin{definition}[Clean]
% A representation $g\in \mathcal{G}$ is {\em clean} iff $g(x) = g(x')$ for all $x\equiv x'$. 
% % A classifier $f\in \F$ is {\em clean} iff $f(x) = f(x')$ for all $x\sim x'$. 
% The set of clean representations is denoted $\G_c$.
% \end{definition}

% Next we prove that solutions to the InfoNCE loss optimized over $\mathcal{G}$ are both clean and satisfy a notion of uniformity in the realizable setting.


%Note that there is an equivalence relation $\sim$ among content variables: $\lc\sim\lc' \implies y(\I(\lc, \ls)) = y(\I(\lc', \ls'))$ for all $y\in \T$. Thus, the equivalence classes consist of sets of images which are classified the same way in {\em all} downstream tasks we would like to consider. 

%Formally we have the following assumption. 

% \textbf{Downstream tasks. }Our downstream tasks consist of classification problems drawn from a (unknown to the learner) set $\T$. Note that there is an equivalence relation $\sim$ among content variables: $\lc\sim\lc' \implies y(\I(\lc, \ls)) = y(\I(\lc', \ls'))$ for all $y\in \T$. Thus, the equivalence classes we get from here consist of sets of images which are classified the same way in {\em all} downstream tasks we would like to consider. We denote the equivalence set for an image $\I(\lc, \ls)$ as $S_{\lc} = \{\I(\lc', \ls')| \lc' \sim \lc\}$ and refer to this set as the \textit{cluster} of image $\I(\lc, \ls)$. We overload the use of the equivalence relation also for images, so $x\sim x'$ if $x = \I(\lc, \ls)$ and $x' = \I(\lc', \ls')$ for $\lc\sim \lc'$. Formally we have the following assumption. 


% as in \cite{haochen2022theoretical}:
% \begin{assumption}[Downstream tasks]\label{assump:downstream}
%     For any downstream task $y$ and all content variables $\lc\sim \lc'$, 
%     \begin{align}
%         \mathbb{P}_{x,x'\sim \I}[y(\I(\lc, \ls))\neq y(\I(\lc', \ls'))] =0.
%     \end{align}
% \end{assumption}




% {\color{red} 
% This bias is formalized as follows:
% \begin{assumption}[Regularity of $\mathcal{F}$ w.r.t. augmentations] \label{assump:spiky}
% For any $f\in \F\setminus \F_c$, $\exists A\in \A$, $x\in \I$ such that $f(A(x))\neq f(x)$.
% \end{assumption}
% \begin{figure}[htb]
% \centering
% \resizebox{5cm}{!}{\input{regularity.tikz}}
% \caption{{\color{red}Illustration of the notion of regularity of Assumption \ref{assump:spiky}. A circular dot represents a natural image, and the L-shaped boxes around each natural image corresponds to its set of augmented images. Note that the purple classifier (horizontal line) splits clusters properly, and also respects augmentations, while the red classifier splits the top cluster in two thereby \textit{necessarily} incurring some inconsistency between a natural image and its augmentation.}}\label{fig:myfigure}
% \end{figure}
% }




% \begin{assumption}[old] \label{assump:spiky-full}
% For any $f\in \mathcal{F}$ and any cluster $C$, let $p(f,C)\coloneqq \min(1-\mathbb{P}_{x_1^- \sim C}[f(x)=1],\mathbb{P}_{x_1^- \sim C}[f(x)=1])$ and $e(f,C)\coloneqq \mathbb{P}_{x \sim \bar{C}, x^+ \sim \mathcal{A}(x)}[f(x)\neq f(x^+)]$. Then for some $\delta\in (0,1]$, a dataset is called $\delta$-spiky with respect to the function class $\mathcal{F}$ if
% \begin{align}
%     \delta p(f,C) \leq e(f,C) \leq 2 p(f,C)
% \end{align}
% for all $f\in \mathcal{F}, C$.
% \end{assumption}






==> Spiky Augmentations/Theory/Downstream.tex <==
\subsection{Downstream Guarantees}
% {\color{red} move after section 4.2? the positive downstream guarantee is only for the realizable setting}

% We first define the space of downstream tasks consistent with our inductive bias assumptions on $\mathcal{F}$. Our main assumption is that downstream tasks label all images from the same cluster alike, hence the clusters are meaningful for downstream performance.
% \begin{assumption}[Meaningful clusters] \label{assump:downstream}
% The set of downstream tasks $\mathcal{T}$ is a subset of $\mathcal{F}_c$.
% \end{assumption}

% Assumption~\ref{assump:downstream} ensures that the inductive bias of the function class is aligned with downstream tasks, which is necessary for any downstream guarantees. Importantly, recall that this bias is inherited by the  representation class $\G$ because each representation in $\G$ consists of concatenated supervised functions.
%
Next we translate the aforementioned representation learning results for $\mathcal{G}$ into downstream performance guarantees. We consider the class of heads consisting of single-layer ReLU neural networks with $m$ neurons.  Formally, $\mathcal{J}_{\text{ReLU}} := \{ \omega_{a,\mathbf{W}, b}: \mathbb{R}^d \rightarrow  \mathbb{R}\; \text{s.t.}\;  \omega_{a,\mathbf{W}, b}(g(x)) = a^\top\text{ReLU}(\mathbf{W}g(x) - b), \; a \in \mathbb{R}^m, \mathbf{W}\in \mathbb{R}^{m \times d}, b \in \mathbb{R}^m  \}$, where $\text{ReLU}(h) = \max(h,0)$. 
% We slightly abuse notation by letting $j\in [m]$ be an indexing over clusters, and defining $\Gamma_j$ as the $j$-th cluster.
\begin{theorem} \label{thm:downstream1} 
% Consider the family of tasks
% $\mathcal{T}_{N}:= \{f \in \mathcal{F}_c : \sum_{j=1}^m \chi\{ y(x)=1 \; \forall\;  x \in \Gamma_j \} \leq N\}$, where $\chi\{\cdot\}$ is the indicator variable. 
Suppose the representation $g^* \in \arg \min_{g \in \mathcal{G}} \mathcal{L}(g)$ under Assumptions \ref{assump:spikyaug} and \ref{assump:realizability}, $\beta > c\log d$ for an absolute constant $c$ and $d>3$. Then for any set of cluster-preserving downstream tasks $\mathcal{T}$, $\mathcal{L}_{\mathcal{T},\J_{\text{ReLU}}}(g^*) = 0$.

% {\color{blue} [KS: $\mathcal{L}_{\mathcal{T},\J_{\text{ReLU}}}$ has not been defined anywhere.][SS: It is in Equation (1), (2)]}


% for any $N \in [m]$ and $\tilde{N} := \max(N,m-N)$, 
% % for any downstream task $y$, there exists a linear head ${w}\in\J_{\text{lin},} :=\mathbb{R}^{ d}$ such that $w^\top g$ achieves zero error, i.e.
% \begin{align}
%      \nonumber
% \end{align}
% or:
% Among all mappings from $m=2^d$ objects to $\mathcal{H}_{d}$, those that map these objects uniformly on the hypercube can express the largest possible number of downstream tasks. 
\end{theorem} 
% In words, $\mathcal{T}_N$ is the set of tasks which positively label images from at most $N$ clusters. 
Theorem \ref{thm:downstream1} shows that any representation learned by minimizing the InfoNCE loss achieves zero downstream error on any task from $\mathcal{F}_c$ with a sufficiently wide two-layer ReLU head.  
% Note that $\mathcal{T}_m = \mathcal{F}_c$, and the maximum number of neurons needed in the head to learn any clean task is $\frac{m}{2}$.



% Next we consider the case in which the heads are two-layer ReLU networks.

% \begin{theorem} \label{thm:downstream1}
%     Let ${U}\in \{-1,1\}^{ 2^d \times d}$ such that each row of $U$ is a unique vertex in $\mathcal{H}_d$. 
% Let $\tilde{g}(x)\coloneqq \text{ReLU}({U}g(x) - (d-1)\mathbf{1})$. Then for any downstream task $\mathcal{T}$, 
% \begin{align}
%     \min_{W \in \mathbb{R}^{r \times 2^d}} \mathcal{L}_{\mathcal{T}}( W, \tilde{g}  ) &= 0
% \end{align}
% \end{theorem}

% lower bound on downstream task error without spiky augmentations

% what if $m \neq 2^d$?

% what if clusters are not the same size?

% example showing how HaoChen assumption/technique can fail on SimCLR? their result follows almost immediately from their assumptions. Ours is more complicated, need to show why. Why is our case hard? would be nice to have positive result for different cluster sizes...

% special case with quantized linear models

% Define the downstream error of a pre-trained representation $g$ on a family of tasks $\mathcal{T}$, with family of heads $\mathcal{W}$.
% \begin{align}
%     \mathcal{L}_{\mathcal{T}, \mathcal{W}}(g) \coloneqq \sup_{T \in \mathcal{T}} \inf_{w \in \mathcal{W}} \mathbb{P}_{x \sim \mathcal{I}}[ w \circ g(x) \neq {T}(x) ].
% \end{align}

{Next, we show that controlling the expressivity of $\mathcal{G}$ is necessary to achieve meaningful downstream performance guarantees. Suppose that instead of optimizing the InfoNCE loss over $\mathcal{G}$, we instead optimized it over a representation class ${\mathcal{G}}_{\star}:= \mathcal{F}_\star^d$ where $\mathcal{F}_\star\coloneqq \{f : {D} \rightarrow \{-1,1\}\}$ consists of all classifiers mapping from images to binary labels.
\begin{theorem} \label{thm:negative}
   Let $\beta > c\log d$ for an absolute constant $c$ and $d>3$. There exists a dataset ${D}$ that satisfies Assumptions \ref{assump:spikyaug} and \ref{assump:realizability} for $\mathcal{G}$, representation $g \in \arg \min_{g'\in \mathcal{G}_{\star}} \mathcal{L}(g')$, and a downstream task $h\in \mathcal{F}_c$ such that 
    % \begin{align}
        $\mathcal{L}_{h,\mathcal{J}_\star}(g) \geq 0.5$,
    % \end{align}
    where $\mathcal{J}_\star= \{\omega : \mathcal{H}_d\rightarrow \{-1,1\} \}$ is the set of all mappings from $\mathcal{H}_d\rightarrow \{-1,1\}$.
\end{theorem}
% \begin{proof} 
% Dataset has two clusters, and there are 2^d vertices. For each vertex, half of the images mapped there by g are from one cluster, the other half are from the other cluster.
% \end{proof}
}


% Can easily show that you get sample complexity gain by a factor of the size of each cluster.

% Say that the task is a singleton. Supervised learner observes 100 samples, gets these samples correct

% We need $d2^d$ samples.
% Next we show that without contrastive pretraining, 
% % supervised learners with arbitrarily large complexity can get arbitrarily large error on even the simplest family of downstream tasks.
% We consider the family of tasks $\mathcal{T}_1$ defined in Theorem \ref{thm:downstream}.


% Define the downstream task error as follows:
% \begin{align}
%     \mathcal{L}_{{T}}(w,g) \coloneqq \mathbb{P}_{x \sim \mathcal{I}}[ w \circ g(x) \neq {T}(x) ].
% \end{align}
% and the downstream 
% \begin{align}
%     \mathcal{L}_{\mathcal{T}}(g) \coloneqq \sup_{T \in \mathcal{T}} \inf_{w \in \mathcal{W}} \mathbb{P}_{x \sim \mathcal{I}}[ w \circ g(x) \neq {T}(x) ].
% \end{align}
% We can learn any task in this family with $O(d2^d)$ samples drawn uniformly from the full set of images. 
% However, supervised learning requires arbitrarily many samples to achieve bounded test accuracy
% \begin{proposition}\label{prop:hard}
% There exists a distribution of  such that any supervised learning algorithm $\text{Alg}$($\cdot$) receiving a set of $n<\infty$ samples $\mathcal{S}$ from a task in $\mathcal{T}_1$ and outputting a hypothesis $h$ achieves worst-case error
% \begin{align}
%     \sup_{f\in \mathcal{T}_1}\mathcal{L}_{y}(\text{Alg}(\mathcal{S})) \geq 0.5
% \end{align}
% with probability 1.
% On the other hand, CL via solving the InfoNCE loss requires  $O(d2^d)$ samples from the downstream task to learn a linear head that achieves zero error w.h.p.
% \end{proposition}

% Theorem 1: with infinitely many samples in the dataset and no assumptions on the clusters (besides equal measure) any supervised learner requires $\infty$ ...unlabelled... samples to achieve $\epsilon$ downstream task error on any task in $\mathcal{T}$, plus $d2^d$ labelled samples, while we can solve them with $d2^d$ labelled samples.

% Theorem 2: If the clusters are Gaussian, Supervised learning requires $.../\epsilon$ samples to learn $\mathcal{T}$... but with our model class? Also Gaussian is not the right way to think about clusters...

% problem is we haven't shown benefit of mapping uniformly to the hypercube in particular. all we really need is a bijection from clusters to some non-colinear set of points.

% The VC dim of F must be large enough . 

% if m > 2^d, clusters can be mapped together, but we can always make d large enough s.t. this shouldn't happen
% if m < 2^d, then we cannot do clean...



==> Spiky Augmentations/Theory/Realizable.tex <==
\section{Results for the Realizable Setting}
\label{sec:realizable}

% \section{SimCLR Leads to Clean Representations}
Our first result shows that when the dataset ${D}$ and representation class $\mathcal{G}$ allow for mapping the data \textit{uniformly} on the hypercube in a \textit{cluster-preserving} manner, then the representation learned by minimizing the InfoNCE loss over $\mathcal{G}$ results in such a mapping. We first formally define the terms \textit{uniform} and \textit{cluster-preserving} below.
 %We show that pretraining using augmentations allows us to learn a representation such that each coordinate respects the augmentations.
% {\color{red} (that is, which is like the green classifier above)}. 
%We refer to such classifiers, and such representations, as \textit{clean}. 

\begin{definition}[Cluster-Preserving]
A {\em cluster-preserving} representation $g \in \mathcal{G}$ is one that for all  {$\mathbf{c} \in C$ } and all $x,x'\in \Gamma_{\mathbf{c}}$, $g(x)= g(x')$.
% A representation $g\in \mathcal{G}$ is {\em clean} iff $g(x) = g(x')$ for all $x\equiv x'$. 
% A classifier $f\in \F$ is {\em clean} iff $f(x) = f(x')$ for all $x\sim x'$. 
\end{definition}

% A \textit{uniform} representation is one in which the push-forward measure onto the hypercube is uniform.
\begin{definition}[Uniform]
A {\em uniform} representation $g\in \mathcal{G}$ satisfies $\Pr_{x\sim {D_\circ}}[g(x)=v]=2^{-d}$ 
for all $v\in \mathcal{H}_d$.
\end{definition}
Next, our results in this section assume a cluster-preserving and uniform representation exists in $\mathcal{G}$.
\begin{assumption}[Realizability]\label{assump:realizability}
    There exists a $g \in \mathcal{G}$ that is both cluster-preserving and uniform.
\end{assumption}
In order for there to exist a representation that is both cluster-preserving and uniform, there must be an integral multiple of $2^d$ clusters in the dataset and they must be balanced.
Before stating our main result, we must prove a key lemma that shows that among all ``clean'' representations, those that minimize the InfoNCE loss are uniform. We define $\mathcal{G}_c \subseteq \mathcal{G}$ as the set of clean representations in $\mathcal{G}$ consisting of $d$ concatenated clean classifiers from $\mathcal{F}_c$. 
% In practice, training on class-unbalanced datasets tends to reduce the performance of models optimized via InfoNCE \citep{assran2022hidden}. 


% {\color{red} We denote $m := m(\mathcal{F}_c, {D})$ as the number of distinct clusters in the dataset.}

% \begin{definition}[Clean]
% A {\em clean} representation $g \in \mathcal{G}_c$ is one that is a concatenation of $d$ clean functions from $\mathcal{F}_c$.
% % A representation $g\in \mathcal{G}$ is {\em clean} iff $g(x) = g(x')$ for all $x\equiv x'$. 
% % A classifier $f\in \F$ is {\em clean} iff $f(x) = f(x')$ for all $x\sim x'$. 
% The set of clean representations is denoted $\G_c$.
% \end{definition}


\begin{lemma}\label{thm:uniform}
     If Assumptions \ref{assump:spikyaug} and \ref{assump:realizability} hold, $\beta > c \log d$ for an absolute constant $c$, $d>3$, and $\ell \geq 1$, then $g^*\in \underset{g\in \mathcal{G}_c}{\arg\min}  \ {\mathcal{L}}(g) $ if and only if $g^*$ is uniform.
\end{lemma}

% {\color{red}
% % At first glance, Lemma \ref{thm:uniform} is not surprising. However, upon further inspection the statement is not as obvious as it may initially seem. 
% Perhaps surprisingly, subtle nuances of the InfoNCE loss are required to prove Lemma \ref{thm:uniform}.
% For example, we can show that when the xx term is removed from the log sum exp in the loss, and $d=3$, minimizer is not uniform... evidence for why this statement is not obvious
% % Consider for example the distribution that maps clusters to the embedded 
% }

\begin{proof}[Proof sketch]
% of Theorem \ref{thm:uniform}]
% {\color{gray}
% By regrouping the terms in \eqref{eq:InfoNCE}, the InfoNCE loss can be written as
% %%%
% \begin{equation}\label{sth}
% {{\mathcal{L}}}(g) =\underset{x,x^+,\{x_i^-\}_{\ell}}{\mathbb{E}} \bigg[  \log\bigg(1+ \sum_{i= 1}^\ell e^{\beta g(x)^\top \left(g(x_{i}^-) - g(x^+)\right)} \bigg)\bigg].
% \end{equation}
% }
Since the optimization problem is over representations composed of clean functions, we know that for all $g\in \mathcal{G}_c$, the term $g(x)^\top g(x^+)$ in the InfoNCE loss is exactly equal to $ d$. Hence, 
% the optimizing $\mathcal{L}(g)$ over $\mathcal{G}_c$ simplifies to minimizing
by regrouping the terms in \eqref{eq:InfoNCE}, the optimization problem simplifies to:
\begin{equation}\label{tilde_loss}
\min_{g\in\mathcal{G}_c}\mathcal{L}(g) = \min_{g\in\mathcal{G}_c}\bigg\{\hat{\mathcal{L}}(g)   \coloneqq \underset{x,x^+,\{x_i^-\}_{\ell}}{\mathbb{E}} \bigg[  \log\bigg(1+ \sum_{i= 1}^\ell e^{\beta g(x)^\top g(x_{i}^-) - \beta d } \bigg)\bigg]\bigg\}
\end{equation}
% over $\mathcal{G}_c$.
By Assumption~\ref{assump:realizability}, at least one uniform representation belongs to the set $\mathcal{G}_c$. We show that it minimizes the loss $\hat{\mathcal{L}}(g)$. To do so, 
we observe that we can think of minimizing $\hat{\mathcal{L}}(g)$ as an optimization with respect to distributions over the hypercube induced by $g$. To better understand this connection, consider the random variable $g(x)$ for $x \sim D_\circ$.
% , where ${D_I}$ is the underlying distribution over images.
Further, denote the corresponding induced distribution over $g(x)$ as $\mathcal{D}_g$, i.e., $\mathcal{D}_g$ is a distribution over the vertices of the hypercube ${\mathcal H}_d$. Letting $y = g(x)$, 
% (and correspondingly, $Y = g(X)$), 
the objective above can now be rewritten in terms of these distributions:
\begin{equation}\label{eq:uniformity}
\min_{\{\mathcal{D}_g: g\in \G_c\}} \bigg\{\tilde{\mathcal{L}}(\mathcal{D}_g) \coloneqq \underset{y,\{y_i^-\}_{\ell}\sim \mathcal{D}_g}{\mathbb{E}}\bigg[  \log\bigg(1+ \sum_{i= 1}^\ell e^{\beta y^\top y_{i}^- - \beta d} \bigg) \bigg]\bigg\}
\end{equation}
% thus our problem is equivalent to:
% $\mathcal{D}_g^* = \argmin_{\{\mathcal{D}_g: g\in \G_c\}} \hat{\mathcal{L}}(\mathcal{D}_g).$

Suppose the the minimizing distribution was not uniform over the hypercube, i.e. for $\mathcal{D}_g^*\in \argmin_{\{\mathcal{D}_g: g\in \G_c\}} \tilde{\mathcal{L}}(\mathcal{D}_g)$, $\mathcal{D}_g^*\ne \mathcal{U}$, where $\mathcal{U} $ is the uniform distribution over the hypercube $\mathcal{H}_d$. 
For any sample
% \footnote{We use capital letters $Y, \{Y_i\}$ to denote random samples, and small letters $y, \{y_i\}$ to denote specific instances.} 
$y, \{y_i\}\sim \mathcal{D}_g$, consider a random walk that starts from this sample and evolves over time. For this random walk, denote the variables at time $t$ by $y^t, \{y_i^t\}$ where $y^t$ (and similarly $y_i^t$ for all $i$), with $y^0 = y$ (correspondingly $y_i^0 = y_i$). The random walk evolves from $y^{t-1}$ to $y^t$ by flipping a uniformly random bit of $y^{t-1}$ with probability $\frac{1}{2}$, and with probability $\frac{1}{2}$, not changing anything; this construction is independent across all samples. We now observe that this construction induces an irreducible, aperiodic Markov chain with uniform stationary distribution over the hypercube. 

With this construction, the critical step in our proof is a surprising ``monotonicity'' property over time:  we show in Appendix \ref{appendix:realizable} that each transition over time decreases the function value as long as $\mathcal{D}_g$ is not uniform. Intuitively, {\em ``blurring'' the distribution $\mathcal{D}_g$ decreases the objective.} 

This result implies that $g$ is a minimizer of the loss ${{\hat{\mathcal{L}}}}(g)$ if and only if $g$ is a uniform representation. 
Consequently, we obtain that among all the representations in $\mathcal{G}_c$, the ones that are uniform minimize the loss in \eqref{eq:uniformity} and the statement of Lemma \ref{thm:uniform} follows. See Appendix~\ref{sec:lemma-prf} for details.
\end{proof}

Using Lemma \ref{thm:uniform}, we show our main result that all minimizers of the InfoNCE loss are uniform and cluster-preserving. 
% {\color{red} The proof also uses the fact that for all representations $g$ that are not cluster-preserving, ${\mathcal{L}}(g)>\hat{\mathcal{L}}(g)$ by Assumption \ref{assump:spikyaug}, where $\hat{\mathcal{L}}$ is defined in \eqref{tilde_loss}. --- MOVE to appendix?} 
To the best of our knowledge, this is the first result characterizing the minimizers of the InfoNCE loss with a finite batch of negative samples. The proof is provided in Appendix \ref{app:uniform-b}. 

\begin{theorem}\label{thm:uniformandclean}
    If Assumptions \ref{assump:spikyaug} and \ref{assump:realizability} hold, and we have $d>3$, $\ell \geq 1$, and $\beta > c \log d$ for an absolute constant $c$, then a representation $g^*\in \mathcal{G}$ is a global minimizer of the loss {${\mathcal{L}}(g) $} optimized over $\mathcal{G}$ if and only if it is uniform and cluster-preserving.
    % , meaning for any $\mathbf{c}\in C$ and any $x,x'\in \Gamma_{\mathbf{c}}\cap D_{\circ}$, $g^*(x)=g^*(x')$. 
    % Additionally, any clean and uniform representation $g$ is a global minimizer of the loss $\mathcal{L}(g)$.
\end{theorem}
% The above result shows that the set of globally optimal solutions of the InfoNCE loss function is equivalent to the set of clean and uniform representations in the realizable setting. 

% The proof relies on the following Theorem, see Appendix~\ref{app:uniform-b} for details.

%Using the above result showing that uniform representations achieve minimal InfoNCE loss among all clean representations (i.e., representations $g$ for which ${\mathcal{L}}(g) = \Tilde{\mathcal{L}}(g)$), {\color{red} we prove the following corollary --- dangling reference here??} by leveraging the fact that for any non-clean $g$, ${\mathcal{L}}(g) >\Tilde{\mathcal{L}}(g)$. We defer the proof to Appendix \ref{app:uniform-b}.


  
% To prove this claim, we first show that among \textit{clean} representations, uniform representations are optimal. We then use this result to show that representations that are not clean are suboptimal.


%\begin{remark} \textbf{(Inductive Bias)} We note that the above result only requires realizability. The discussion on inductive bias in Section~\ref{sec:cluster-bias} and the corresponding Assumption~\ref{assump:downstream} is required only when we compose this learned representation with a head for downstream tasks, discussed below.\end{remark}

% \begin{proof}[Proof of Theorem \ref{thm:uniformandclean}] Recall the definitions of the functions ${{\mathcal{L}}}(g)$ in \eqref{sth} and ${{\tilde{\mathcal{L}}}}(g)$ in \eqref{tilde_loss}. Note that since we always have $g(x)^\top g(x^+) \le d$, we can argue that for any $g$ we have $\mathcal{L}(g)\ge \tilde{\mathcal{L}}(g)$. Indeed, the equality holds when $g$ is a clean representation. Moreover, for any non-clean representation $g$, we know that  there exists at least one image $x$ for which its representation $g(x)$ is not exactly aligned with the representation of one of its augmented images. Therefore, the first term of the InfoNCE loss, i.e., $-\underbrace{ \beta \mathbb{E}_{x,x^+} [g(x)^\top g(x^+) ]}_{\text{alignment}} $, for that representation would be strictly larger than $- \beta d$. Hence, for non-clean $g$ we have $\mathcal{L}(g)> \tilde{\mathcal{L}}(g)$.

% Moreover, according to the result of Lemma \ref{thm:uniform}, we know that the minimizer of the loss function $\tilde{\mathcal{L}}$ is a uniform representation, thus for any non-uniform representation $g'$ and uniform representation $g''$ we have $\tilde{\mathcal{L}}(g')> \tilde{\mathcal{L}}(g'')$.

% %Consider the related loss given below, where the positive inner product is replaced by its upper bound: 
% %\begin{equation}\label{eq:Ltilde}
% %\tilde{\mathcal{L}}(g) \coloneqq \underset{x,\{x_i^-\}_{\ell}}{\mathbb{E}}[  \log(1+ \sum_{i= 1}^\ell e^{\beta \left(g(x)^\top g(x_{i}^-) - d\right)} ) ]
% %\end{equation}

% Considering these two observations, we show that a clean uniform representation denoted by $g^*$ is an optimal solution of the loss ${\mathcal{L}}$. We consider the following two cases:

% \textbf{Case 1:} If the representation $g'$ is not clean then we have
%  \begin{align}
%        {\mathcal{L}}(g') &\stackrel{(a)}{>} \tilde{\mathcal{L}}(g') \stackrel{(b)}{\geq} \tilde{\mathcal{L}}(g^*) \stackrel{(c)}{=}{\mathcal{L}}(g^*)  \nonumber
%    \end{align}
%     where $(a)$ holds with strict inequality since $g'$ is not clean, $(b)$ holds as $g^*$ with a uniform distribution is an optimal solution of  $\tilde{\mathcal{L}}$, and $(c)$ holds because $g^*$ is clean.
    
% \textbf{Case 2:} If the representation $g'$ is not uniform then we have 
%  \begin{align}
%        {\mathcal{L}}(g') &\stackrel{(a)}{\geq } \tilde{\mathcal{L}}(g') \stackrel{(b)}{>} \tilde{\mathcal{L}}(g^*) \stackrel{(c)}{=}{\mathcal{L}}(g^*)  \nonumber
%    \end{align}
%       where $(a)$ holds based on the definitions of ${\mathcal{L}}$ and $\tilde{\mathcal{L}}$,  $(b)$~holds since $g'$ is not uniform  and $g^*$ is uniform, and $(c)$~holds because $g^*$ is clean.

% Combining these two cases, we obtain that the representation $g^*$ minimizes $\mathcal{L}(\cdot)$ if and only if $g^*$ is clean and uniform.
% % Suppose that $g'\in \arg \min_{g \in \mathcal{G}} \mathcal{L}(g)$ is not clean.
%    % Theorem \ref{thm:uniform} implies that all $\tilde{g} \in \arg \min_{g \in \mathcal{G}} \tilde{\mathcal{L}}(g)$ are uniform.  Further,
%    % Assumption \ref{assump:spiky} implies that for any representation $g \in \mathcal{G}$ that is not clean,  ${\mathcal{L}}(g) > \tilde{\mathcal{L}}(g)$, whereas ${\mathcal{L}}(g) = \tilde{\mathcal{L}}(g)$ for all clean $g\in \mathcal{G}$. 
%  %  Let $g*$ be clean and uniform and suppose $g'\in \arg \min_{g \in \mathcal{G}} \mathcal{L}(g)$ is  not clean and/or not uniform. Then 
%  %  \begin{align}
%   %     {\mathcal{L}}(g') &\stackrel{(a)}{\geq} \tilde{\mathcal{L}}(g') \stackrel{(b)}{\geq} \tilde{\mathcal{L}}(g^*) \stackrel{(c)}{=}{\mathcal{L}}(g^*)  \nonumber
%  %  \end{align}
% \end{proof}


% A few comments are in order to interpret Theorem \ref{thm:uniformandclean} and Lemma \ref{thm:uniform}.
% \begin{itemize}
% \item \textbf{Solutions to SimCLR have good downstream properties.} as we will show below.
%     \item \textbf{Scaling of allowed number of clusters.}
%     \item \textbf{Why proving Theorem \ref{thm:uniform} is hard.} example with clusters optimally mapped to the 2-hypercube embedded in the 3-hypercube to show that it is not obvious that the uniform distribution over the hypercube is best (proof in appendix)
% \end{itemize}

==> Spiky Augmentations/Theory/UniformityProofSketch.tex <==
% \section{Proof Sketch for Theorem \ref{thm:uniform}}


